From Realizability Modulo Theories to Synthesis Modulo Theories Part 1: Dynamic approach

Reactive synthesis is the process of using temporal logic specifications in LTL to generate correct controllers, but its use has been restricted to Boolean specifications. Recently, a Boolean abstraction technique allows to translate LTL T specifications that contain literals in theories into equi-realizable LTL specifications. However, no synthesis procedure exists yet. In synthesis modulo theories, the system to synthesize receives valuations of environment variables in a first-order theory T and outputs valuations of system variables from T . In this paper, we address how to syntheize a full controller using a combination of the static Boolean controller obtained from the Booleanized LTL specification together with dynamic queries to a solver that produces models of a satisfiable existential formulae from T . This is the first method that realizes reactive synthesis modulo theories.

==> figures/latex/definitions.tex <==
\newcommand{\Terms}{\mathcal{T}}


%
\newcommand{\Str}{\mathcal{S}} \newcommand{\StrDesc}{\Rightarrow}
\newcommand{\StrReaches}{\StrDesc^*} \newcommand{\Desc}{\mapsto}
\newcommand{\DirDesc}{\rightarrow}
%
\newcommand{\RecDesc}{\twoheadrightarrow}
\newcommand{\AnyDesc}{\rightsquigarrow}
\newcommand{\AlphaDesc}{\dasharrow}
\newcommand{\ALPHADesc}[1]{\stackrel{#1}\dasharrow}
\newcommand{\Reaches}{\AnyDesc^*}
\newcommand{\Class}[1]{\ensuremath{[#1]}}
\newcommand{\EqSite}[2]{#1\equiv_{\Reactors}#2}
\newcommand{\LiveP}{\textsc{Live-P}\xspace}
\newcommand{\SchemaP}{\textsc{Schema-P}\xspace}
\newcommand{\BadP}{\textsc{Bad-P}\xspace} \newcommand{\INVname}{\phi}
\newcommand{\INV}{\ensuremath{\INVname}\xspace}
%
\newcommand{\INVnext}[2]{\ensuremath{\INVname_{#1}^{({#2})}}}
\newcommand{\INVclause}[1]{\ensuremath{\INVname[#1]}}
\newcommand{\INVnextclause}[3]{\ensuremath{\INVname_{#1}^{({#2})}[#3]}}
\newcommand{\React}[1]{\text{react}(#1)} \newcommand{\bisim}{\approx}
\newcommand{\Await}{\mathbf{await}} \newcommand{\When}{\mathbf{when}}
\newcommand{\Do}{\mathbf{do}} \newcommand{\Dec}{\texttt{--}}
\newcommand{\Inc}{\texttt{++}} \newcommand{\Width}{6em}
\newcommand{\Type}[1]{\hspace{-0.2em}:\hspace{-0.2em}#1} %
\newcommand{\LHeight}{\textit{lh}} \newcommand{\Height}{\textit{h}}
\newcommand{\owise}{\text{otherwise}}
\newcommand{\EmptyP}{\textsc{Empty-P}\xspace}
\newcommand{\AdequateP}{\textsc{Adequate-P}\xspace}
\newcommand{\BasicP}{\textsc{Basic-P}\xspace}
\newcommand{\BasicPRec}{\textsc{BasicRec-P}\xspace}
\newcommand{\EfficientP}{\textsc{Efficient-P}\xspace}
\newcommand{\kEfficientP}{\ensuremath{k}\textsc{-Efficient-P}\xspace}
\newcommand{\jEfficientP}{\ensuremath{j}\textsc{-Efficient-P}\xspace}
\newcommand{\Proc}{\mathcal{P}}
\newcommand{\WaitOnConnection}{\emph{WaitOnConnection}\xspace}
\newcommand{\WaitOnReactor}{\emph{WaitOnReactor}\xspace}
\newcommand{\process}{task\xspace}
\newcommand{\emprocess}{\emph{task}\xspace}
\newcommand{\processes}{tasks\xspace}
\newcommand{\emprocesses}{\emph{tasks}\xspace}
\newcommand{\subprocess}{sub-task\xspace}
\newcommand{\emsubprocess}{\emph{sub-task}\xspace}
\newcommand{\subprocesses}{sub-tasks\xspace}
\newcommand{\abs}[1]{\lvert #1 \rvert}
\newcommand{\AllocName}{\textit{alloc}}
\newcommand{\Alloc}[1]{\textit{alloc\textup{(}[#1]\textup{)}}}
\newcommand{\AllocBigger}[1]{\textit{alloc.bigger\textup{(}#1\textup{)}}}
\newcommand{\AllocInc}[1]{\textit{alloc.inc\textup{(}#1\textup{)}}}
\newcommand{\AllocDec}[1]{\textit{alloc.dec\textup{(}#1\textup{)}}}
\newcommand{\p}[1]{\ensuremath{a[#1]}}
%
\newcommand{\Pplus}[1]{\ensuremath{A[#1]}}
\newcommand{\pnext}[2]{\ensuremath{a'_{#1}[#2]}}
\newcommand{\Pplusnext}[2]{\ensuremath{A'_{#1}[#2]}} %
\newcommand{\En}[2]{\mathit{En}_{#1}(#2)} %
\newcommand{\In}[2]{\mathit{In}_{#1}(#2)} %
\newcommand{\Out}[2]{\mathit{Out}_{#1}(#2)} %
\newcommand{\Pres}[1]{\mathit{pres}({#1})}
\newcommand{\Log}[1]{\mathit{log}\;#1}
\newcommand{\EnNm}{\ensuremath{\mathit{En}}}
\newcommand{\EnName}{\EnNm\xspace} 
%
\newcommand{\InNm}{\ensuremath{\mathit{In}}}
\newcommand{\InName}{\InNm\xspace} 
%
\newcommand{\OutNm}{\ensuremath{\mathit{Out}}}
\newcommand{\OutName}{\OutNm\xspace}
%
\newcommand{\StateSpace}{\ensuremath{\mathcal{S}}}
\newcommand{\phiStates}{\ensuremath{\INV\text{-states}}\xspace}
\newcommand{\phiState}{\ensuremath{\INV\text{-state}}\xspace}
\newcommand{\AlgName}{\textsc{Minimal}}
\newcommand{\Alg}[2]{\ensuremath{\AlgName(#1,#2)}}

%

\newcommand{\LangInf}{\Lang_\text{inf}} %
\newcommand{\ArrowType}{\SelectTips{cm}{}} %



 \newcommand{\SetCategory}{\mathcal{S}\textit{et}}


\newcommand{\RLTL}{RLTL\xspace}
\newcommand{\LTL}{LTL\xspace}
\newcommand{\MuCalculus}{\ensuremath{\mu\text{-calculus}}}
%
\newcommand{\nuTL}{\ensuremath{\nu\text{TL}}}

\newcommand{\semInf}[1]{\Lang_\omega(#1)}
\renewcommand{\sem}[1]{\Lang(#1)}
\newcommand{\Aut}[1]{\ensuremath{\mathcal{#1}}}
\newcommand{\AutA}{\Aut{A}}

\newcommand{\Prop}{\textit{Prop}}


\newcommand{\PreL} [1]{\ensuremath{\!\!\phantom{.}^{-}#1}}
\newcommand{\PostL}[1]{\ensuremath{#1^{-}}}
\newcommand{\PreR} [1]{\ensuremath{\phantom{.}^{+}#1}}
\newcommand{\PostR}[1]{\ensuremath{#1^{+}}}
\newcommand{\NoMove}[1]{{\ensuremath{#1^{0}}}}
\newcommand{\BasicProp}{\Bool(\Prop)}
\newcommand{\BminusProp}{\PostL{\Bool}(\Prop)}
\newcommand{\Segment}[3]{(#1,#2,#3)}
\newcommand{\Inv}[1]{\ensuremath{#1^{-1}}}
%\newcommand{\Segment}[3]{#1[#2,#3]}
\newcommand{\Pointed}[2]{(#1,#2)}
%\newcommand{\Pointed}[2]{#1^{#2}}
\newcommand{\NotFirst}{\ensuremath{\mathit{notfirst}}}
\newcommand{\First}{\ensuremath{\mathit{first}}}

\newcommand{\modelsLTL}{\models_{\textsc{LTL}}}



==> figures/latex/figures/figures.tex <==
%\UseComputerModernTips

\newcommand{\ST}[1]{**[F-]{\texttt{#1}}}
\newcommand{\PROC}[1]{**[F-:<40pt>]{\textit{#1}}}
\newcommand{\EmbeddedAppsST}{
  \ST{\begin{tabular}{c}Embedded\\Application\\(C sources)\end{tabular}}}
\newcommand{\DirectST}{
  \PROC{\begin{tabular}{c}\phantom{A}\\\Direct\\\phantom{a} \end{tabular}}}
\newcommand{\InstrumentedSourcesST}{
  \ST{\begin{tabular}{c}Instrumented\\Annotated\\C sources\end{tabular}}}
\newcommand{\RuntimeManagerST}{
  \PROC{\begin{tabular}{c}\Direct\\Runtime\\Manager\end{tabular}}}
\newcommand{\CompileLinkST}{
  \PROC{\begin{tabular}{c}Compile\\Link\end{tabular}}}
\newcommand{\EmbeddedAppExecST}{
  \ST{\begin{tabular}{c}Embedded\\Application\\(executable)\end{tabular}}}




\newcommand{\FlowFig}{
  {\scriptsize
   \xymatrix@W=4.5em @H=4em @R=0em @C=3em {
     & & \RuntimeManagerST \ar[dr] & & \\
     \EmbeddedAppsST\ar[r] & \DirectST\ar[ur]\ar[dr] & & 
     \CompileLinkST \ar[r] & \EmbeddedAppExecST\\
     & & \InstrumentedSourcesST \ar[ur] & & \\
   }}
}
  
\newcommand{\Queue}[1]{**[F-]{\textrm{#1}}}
\newcommand{\Proc}[1]{**[F-:<50pt>]{\textit{#1}}}
%\newcommand{\Proc}[1]{*++[o][F-]{\textit{#1}}}

\newcommand{\AdhocFig}{
  {\scriptsize
   \xymatrix@W=4em @H=1.5em @R=1.3em @C=5em {
                              & \Proc{user}\ar[dl] & \Queue{user}\ar[l] &  \\
     \Queue{input}\ar[r] & \Proc{router}\ar[ur]\ar[r]\ar[dr] & \Queue{broadcast}\ar[dr] & \\
     \Proc{generator}\ar[u] & \Proc{sender}\ar[ur] & \Queue{output}\ar[l] & \Proc{delay}\ar[l]
  }
}}

==> figures/latex/macros.tex <==
%%%% LTL Symbols %%%%%
\makeatletter
\DeclareFontFamily{OMX}{MnSymbolE}{}
\DeclareSymbolFont{MnLargeSymbols}{OMX}{MnSymbolE}{m}{n}
\SetSymbolFont{MnLargeSymbols}{bold}{OMX}{MnSymbolE}{b}{n}
\DeclareFontShape{OMX}{MnSymbolE}{m}{n}{
    <-6>  MnSymbolE5
   <6-7>  MnSymbolE6
   <7-8>  MnSymbolE7
   <8-9>  MnSymbolE8
   <9-10> MnSymbolE9
  <10-12> MnSymbolE10
  <12->   MnSymbolE12
}{}
\DeclareFontShape{OMX}{MnSymbolE}{b}{n}{
    <-6>  MnSymbolE-Bold5
   <6-7>  MnSymbolE-Bold6
   <7-8>  MnSymbolE-Bold7
   <8-9>  MnSymbolE-Bold8
   <9-10> MnSymbolE-Bold9
  <10-12> MnSymbolE-Bold10
  <12->   MnSymbolE-Bold12
}{}

\let\llangle\@undefined
\let\rrangle\@undefined
\DeclareMathDelimiter{\llangle}{\mathopen}%
                     {MnLargeSymbols}{'164}{MnLargeSymbols}{'164}
\DeclareMathDelimiter{\rrangle}{\mathclose}%
                     {MnLargeSymbols}{'171}{MnLargeSymbols}{'171}
\makeatother

% \newcommand{\mymid}{\mathbin{\mid}}
% \newcommand{\Power}[3]{{#2}\!\mymid\!{#1}\rangle\!\rangle{#3}}
% \newcommand{\WeakPower}[3]{{#2}\mymid\!{#1}\rangle{#3}} %warning: not dual power!!
% \newcommand{\PowerSub}[3]{{#2}\mymid{#1}\rangle\!\rangle{#3}}
% \newcommand{\WeakPowerSub}[3]{{#2}\mymid{#1}\rangle{#3}} %warning: not dual power!!

\newcommand{\Always}{\LTLsquare}
%\newcommand{\Always}{\mathbf{G}}
\newcommand{\Event}{\LTLdiamond}
\newcommand{\Eventually}{\Event}
\newcommand{\Next}{\LTLcircle}
\newcommand{\PrevLTL}{\LTLcircleminus}
\newcommand{\Previously}{\Prev}
\newcommand{\PrevNoFirst}{\LTLcircletilde}
\newcommand{\Before}{\PrevNoFirst}
\newcommand{\HasAlwaysBeen}{\LTLsquareminus}
\newcommand{\SoFar}{\HasAlwaysBeen}
\newcommand{\Once}{\LTLdiamondminus}
\newcommand{\Since}{\mathbin{\mathcal{S}}}
\newcommand{\BackTo}{\mathbin{\mathcal{B}}}
\newcommand{\WeakPrev}{\LTLcircletilde}
\newcommand{\UNTIL}{\mathbin{\mathcal{U}}}
\newcommand{\WaitFor}{\mathbin{\mathcal{W}}}


%\newenvironment{proposition}{\theoremlike{Proposition}}{\par\medskip}

\newcommand{\val}[1]{\ensuremath{[\![ #1 ]\!]}}

\newcommand{\der}[1]{\ensuremath{\;\;{\mathop{{ %
            \longrightarrow}}\limits^{{#1}}}\!}\;\;} %

\newcommand{\Der}[1]{\ensuremath{\rightarrow_{#1}}} %
\newcommand{\notDer}[1]{\ensuremath{\not\rightarrow_{#1}}} %
%\newcommand{\notDer}[1]{\ensuremath{\;\;\not\rightarrow_{#1}\;\;}} %


\newcommand \tpl[1]{\langle #1 \rangle}


\newcommand{\LTL}{\textsf{LTL}\xspace}
\newcommand{\ForSpec}{\textsf{ForSpec}\xspace}

\newcommand{\SVA}{\textsf{SVA}\xspace}
\newcommand{\VLTL}{\textsf{VLTL}\xspace}
\newcommand{\RLTL}{\textsf{RLTL}\xspace}
%\newcommand{\RE}{\textsf{RE}\xspace}
\newcommand{\NVPA}{\textsf{NVPA}\xspace}
\newcommand{\VPA}{\textsf{VPA}\xspace}
\newcommand{\NFA}{\textsf{NFA}\xspace}
\newcommand{\VPL}{\textsf{VPL}\xspace}
\newcommand{\CARET}{\textsf{CaRet}\xspace}
\newcommand{\VPLs}{\textsf{VPL}s\xspace}
\newcommand{\VRL}{\textsf{VRL}\xspace}
\newcommand{\VRE}{\textsf{VRE}\xspace}
\newcommand{\EMSO}{\textsf{MSO$_{\mu}$}\xspace}
\newcommand{\MSO}{\textsf{MSO}\xspace}
\newcommand{\FO}{\textsf{FO}\xspace}
\newcommand{\EFO}{\textsf{FO}$_{\mu}$\xspace}
\newcommand{\XML}{\textsf{XML}\xspace}
%\newcommand{\ETL}{\textsf{ETL}\xspace}
\newcommand{\PDL}{\textsf{PDL}\xspace}
\newcommand{\AJA}{\textsf{AJA}\xspace}
\newcommand{\AJT}{\textsf{AJT}\xspace}
\newcommand{\SAJA}{\textsf{SAJA}\xspace}
\newcommand{\MAJA}{\textsf{MAJA}\xspace}
\newcommand{\AFA}{\textsf{AFA}\xspace}
\newcommand{\AVPA}{\textsf{AVPA}\xspace}
\newcommand{\PSL}{\textsf{PSL}\xspace}

\newcommand{\NWTL}{\textsf{NWTL}\xspace}
\newcommand{\NWTLPLUS}{\textsf{NWTL}$^{+}$\xspace}


\newcommand{\TWOEXPTIME}{\textsf{2-EXPTIME}\xspace}
\newcommand{\EXPTIME}{\textsf{EXPTIME}\xspace}
\newcommand{\PTIME}{\textsf{PTIME}\xspace}

\newcommand{\WM}{\ensuremath{\mathit{WM}}}
\newcommand{\MR}{\ensuremath{\mathit{MR}}}
\newcommand{\MC}{\ensuremath{\mathit{MC}}\xspace}
\newcommand{\SWM}{\ensuremath{\mathit{MWM}}\xspace}
\newcommand{\Pu}{\ensuremath{\mathcal{P}}}
\newcommand{\Lang}{\ensuremath{\mathcal{L}}}
\newcommand{\Au}{\ensuremath{\mathcal{A}}}
\newcommand{\Gam}{\ensuremath{\mathcal{G}}}
\newcommand{\Tu}{\ensuremath{\mathcal{T}}}
\newcommand{\Stratum}{\ensuremath{\mathcal{S}}}
\newcommand{\RejMain}{\ensuremath{\bot_\MainStates}}
\newcommand{\RejSec}{\ensuremath{\bot_\SecStates}}

%%%%
%%%% The following three macros are confusing with MainStates and SecStates
%%%%
\newcommand{\Msubst}{$M$-substitution\xspace} % M-substitution CHANGE FONT
\newcommand{\Mclosure}{$M$-closure\xspace}    %
\newcommand{\Sclosure}{$S$-closure\xspace}    %

\newcommand{\Region}{\ensuremath{\mathcal{R}}}

%\newcommand{\MainStates}{\ensuremath{\textit{M}}}
%\newcommand{\MainStates}{\ensuremath{M}}
\newcommand{\MainStates}{\ensuremath{\mathsf{M}}}
%\newcommand{\SecStates}{\ensuremath{\textit{S}}}
%\newcommand{\SecStates}{\ensuremath{S}}
\newcommand{\SecStates}{\ensuremath{\mathsf{S}}}
%\newcommand{\FamStratum}{\ensuremath{\mathfrak{F}}}
\newcommand{\FamStratum}{\ensuremath{\mathsf{F}}}
\newcommand{\Acc}{\ensuremath{\textit{Acc}}}
\newcommand{\Inf}{\ensuremath{\textit{Inf}}}
\newcommand{\SF}{\ensuremath{\textit{SF}}}
\newcommand{\Model}{\ensuremath{\textit{X}}}



\newcommand{\Stilde}{\widetilde{\Sigma}\xspace}
\newcommand{\Scall}{\Sigma_{\mathit{call}}}
\newcommand{\call}{{\mathit{call}}}
\newcommand{\ret}{{\mathit{ret}}}
\newcommand{\intA}{{\mathit{int}}}
\newcommand{\Sret}{\Sigma_{\mathit{ret}}}
\newcommand{\Sint}{\Sigma_{\mathit{int}}}

\newcommand{\Nat}{\mathbb{N}}



\newcommand{\SubstOp}[1]{\mathrel{\curvearrowleft_{#1}}}
\newcommand{\SubstBox}{\SubstOp{\Box}}
\newcommand{\MClos}[2]{#1^{\SubstOp{#2}}}
\newcommand{\LangClos}{\MClos{\Lang}{\Box}}
\newcommand{\SClos}[2]{{#1}^{\circlearrowleft_{#2}}}
\newcommand{\SClosure}[1]{\SClos{#1}{\Box}}
\newcommand{\LangSClos}{\SClos{\Lang}{\Box}}

\newcommand{\caller}{\mathsf{c}}
\newcommand{\down}{\mathsf{+}}
\newcommand{\abs}{\mathsf{a}}
\newcommand{\absExt}{\mathsf{ea}}
\newcommand{\PosBool}{\ensuremath{\mathcal{B}^{+}}}

%\newcommand{\dirUp}{\ensuremath{\uparrow}}
\newcommand{\dirUp}{\ensuremath{\leftarrow}}
%\newcommand{\dirDown}{\ensuremath{\downarrow}}
\newcommand{\dirDown}{\ensuremath{\rightarrow}}
%\newcommand{\dirUpAbs}{\ensuremath{\uparrow^{\abs}}}
\newcommand{\dirUpAbs}{\ensuremath{\curvearrowleft}}
%\newcommand{\dirDownAbs}{\ensuremath{\downarrow_{\abs}}}
\newcommand{\dirDownAbs}{\ensuremath{\curvearrowright}}
%\newcommand{\dirDownAbsExt}{\ensuremath{\downarrow_{\absExt}}}
%\newcommand{\dirDownAbsExt}{\ensuremath{\curvearrowright_{\mkern-15.2mu\raisebox{.30em}{$\phantom{.}_{\bullet}$}}}}
\newcommand{\dirDownAbsExt}{\ensuremath{\curvearrowright_{\mkern-8.5mu{\bullet}}}}
%\newcommand{\dirUpAbsExt}{\ensuremath{\uparrow^{\absExt}}}
%\newcommand{\dirUpAbsExt}{\ensuremath{\curvearrowleft_{\mkern-30.2mu\raisebox{.30em}{$\phantom{.}_{\bullet}$}}}}
\newcommand{\dirUpAbsExt}{\ensuremath{\phantom{.}_\bullet{\mkern-8.2mu\curvearrowleft}}}

\newcommand{\DIR}{\textit{DIR}}
\newcommand{\Trans}{\texttt{t}}
\newcommand{\Moves}{\textit{Moves}}
%\newcommand{\dir}{\textit{dir}}
\newcommand{\SUCC}{\mathsf{succ}}
\newcommand{\NULL}{\mathsf{\bot}}
\newcommand{\acc}{\textit{acc}}
\newcommand{\rej}{\textit{rej}}
\newcommand{\rank}{\textit{rank}}
\newcommand{\widt}{\textit{width}}

\newcommand{\DefinedAs}{\,\stackrel{\text{def}}{=}\,}

%\newcommand{\DefOR}{\ensuremath{\;\;\;\big|\;\;\;}}
\newcommand{\DefORmini}{\ensuremath{\;\big|\;}}

\newcommand{\details}[1]{}

%%%%%% Temporal Modalities %%%%%%%%%%%%%%

\newcommand{\true}{\ensuremath{\textup{\texttt{true}}}}
\newcommand{\false}{\ensuremath{\textup{\texttt{false}}}}
\newcommand{\Power}[3]{\mathrel{{#1}|{#2}\rrangle{#3}}}
\newcommand{\Norm}[1]{\ensuremath{\|{#1}\|}}
\newcommand{\WeakPower}[3]{\mathrel{{#1}|{#2}\rangle{#3}}}
\newcommand{\PastPower}[3]{\mathrel{{#1}\llangle{#2}|{#3}}}
\newcommand{\PastWeakPower}[3]{\mathrel{{#1}\langle{#2}|{#3}}}
%\newcommand{\Next}{\ensuremath{\bigcirc}}
\newcommand{\Seq}{\ensuremath{;}}
%\newcommand{\Previous}{\ensuremath{{\mathrlap{\bigcirc}\,\minus\,}}}
\newcommand{\Previous}{\Prev}
%\newcommand{\until}{{\sf U}}
\newcommand{\until}{\Until}
%\newcommand{\since}{{\sf S}}
\newcommand{\since}{\Since}
%\newcommand{\sometimes}{\lozenge}
%\newcommand{\always}{\square}
\newcommand{\always}{\Always}

\newcommand{\comp}[1]{\ensuremath{\overline{#1}}} % complement automaton
\newcommand{\dual}[1]{\ensuremath{\widetilde{#1}}} % dualization

\newcommand{\Outcm}{c\,b\,r}
\newcommand{\UOutcm}{\underline{\Outcm}}

\newenvironment{changemargin}[2]{%
  \begin{list}{}{%
    \setlength{\topsep}{0pt}%
    \setlength{\leftmargin}{#1}%
    %\setlength{\footnotewidth}{#1}%
    \setlength{\rightmargin}{#2}%
    \setlength{\textheight}{21cm}%
   \setlength{\topmargin}{0cm}
   \setlength{\listparindent}{\parindent}%
    \setlength{\itemindent}{\parindent}%
    \setlength{\parsep}{\parskip}%
  }
  \item[]}{\end{list}}


\newcommand{\push}{\textit{push}}
\newcommand{\Regions}{\ensuremath{\textit{REG}}}
\newcommand{\pop}{\textit{pop}}
%\newcommand{\pending}{\ensuremath{\texttt{pending}}}

\newcommand{\Bu}{\ensuremath{\textsf{B}}}
\newcommand{\Co}{\ensuremath{\textsf{C}}}

\newcommand{\alphaANY}{\ensuremath{\alpha_{\mathit{ONE}}}}

%%%% ATTENTION HERE: DON'T USE OLD DEFINITION IN FSTTCS CLASS iS treated as a section %%%%
\newcommand{\myparagraph}[1]{\paragraph{\textup{\textbf{#1}}}}
%\newcommand{\myparagraph}[1]{\noindent\textbf{#1}}

\newcommand{\myparagraphApp}[1]{\vspace{0.5em}\noindent\textup{\textbf{#1}}}

\newcommand{\qin}{\ensuremath{q_{\textit{in}}}}

% MINE
\newcommand{\striver}{\textsf{Striver}\xspace}

\newcommand{\tessla}{TeSSLa\xspace}

\newcommand{\reserved}[1]{\ensuremath{\mathit{#1}}\xspace}
\newcommand{\Syntax}[1]{\keyword{#1}}


\newcommand{\wakeUpTicks}{\reserved{ticks^*}}
\newcommand{\ticks}{\reserved{ticks}}

\newcommand{\caseof}[1]{\mathtt{case}~#1~\mathtt{of}}
%\newcommand{\IF}{\mathtt{if}}  %% Defined in algorithmic
%\newcommand{\THEN}{\mathtt{then}}
%\newcommand{\ELSE}{\mathtt{else}}
%\newcommand{\ELSIF}{\mathtt{elsif}}

\newcommand{\IfThenElse}[3]{\mathtt{if}~#1~\mathtt{then}~#2~\mathtt{else}~#3}

\newcommand{\IntoP}{\mathrel{\rightharpoondown}}


\newcommand{\Vc}[1]{\ensuremath{\langle #1 \rangle}}

\newcommand{\default}{\reserved{default}}
\newcommand{\lift}{\reserved{lift}}
\newcommand{\delay}{\keyword{delay}}
\newcommand{\SHIFT}{\keyword{shift}}

%\newcommand{\at}{\keyword{delayLast}}
\newcommand{\at}{\keyword{at}}

\newcommand{\PrevVal}{\reserved{valprev}}
%\newcommand{\Prev}{\reserved{tprev^{\leftarrow}}}
%\newcommand{\Prev}{\reserved{prev}}
%\DeclareMathOperator*{\prevOp}{\reserved{prev}}
\DeclareMathOperator{\prevOp}{\reserved{prev}}
\DeclareMathOperator{\succOp}{\reserved{succ}}
%\newcommand{\Prev}{\ensuremath{\ensuremath{\reserved{prev}}\limits{\leq}}}
\newcommand{\Prev}{\ensuremath{\prevOp\limits_{<}}}
\newcommand{\PrevEqVal}{\reserved{valprev_\circ}}
%\newcommand{\PrevEq}{\reserved{tprev}}
%\newcommand{\PrevEq}{\reserved{prev_\circ}}
\newcommand{\PrevEq}{\ensuremath{\prevOp\limits_{\leq}}}
\newcommand{\Succ}{\ensuremath{\succOp\limits_{>}}}
\newcommand{\SuccEqVal}{\reserved{valsucc_\circ}}
%\newcommand{\SuccEq}{\reserved{tsucc}}
%\newcommand{\SuccEq}{\reserved{succ_\circ}}
\newcommand{\SuccEq}{\ensuremath{\succOp\limits_{\geq}}}

\newcommand{\PrevS}{\Syntax{\ll}}
%\newcommand{\PrevEqS}{\Syntax{<\sim}}
%\newcommand{\PrevEqS}{\Syntax{<\text{\raisebox{10ex}{$\sim$}}}}
%\newcommand{\PrevEqS}{\ensuremath{\mathrel{\ooalign{$<$\cr\hidewidth\raise{20ex}\hbox{$\sim$}\cr}}}}
\newcommand{\PrevEqS}{\ensuremath{\mathrel{\ooalign{$<$\cr\hidewidth\raisebox{-1.2ex}{$\sim$}\cr}}}}
\newcommand{\SuccS}{\Syntax{\gg}}
%\newcommand{\SuccEqS}{\Syntax{\sim>}}
\newcommand{\SuccEqS}{\ensuremath{\mathrel{\ooalign{$>$\cr\hidewidth\raisebox{-1.2ex}{$\sim$}\cr}}}}
\newcommand{\setS}[1]{\Syntax{\{} #1 \Syntax{\}}}
\newcommand{\valS}[1]{\textsf{(}#1\textsf{)}}
\newcommand{\Ticks}{\keyword{ticks}}
\newcommand{\ticksS}{\keyword{ticks}}
\newcommand{\Union}{\mathrel{\textsf{U}}}
%\newcommand{\delaySym}{\Syntax{delay}}
%\newcommand{\delayS}[1]{\delaySym{}(#1)}
\newcommand{\delayS}[1]{\delay{}(#1)}
%\newcommand{\atSym}{\Syntax{at}}
%\newcommand{\atS}[1]{\atSym{}(#1)}
\newcommand{\atS}[1]{\at{}(#1)}


\newcounter{Problem} \setcounter{Problem}{0}

\newcommand{\Prob}{\addtocounter{Problem}{1}\noindent\paragraph{\textbf{Problem
      \#\theProblem}}}

\newcommand{\Abs}[1]{\ensuremath{#1^\#\xspace}}

\newcommand{\LET}{\mathtt{let}}
\newcommand{\MAX}{\ensuremath{\mathit{max}}}
%\newcommand{\DefOr}{\ensuremath{\hspace{1em}\big|\hspace{1em}}}


\newcommand{\tprev}{\ensuremath{t_{\textit{prev}}}}

\newcommand{\Tstar}{\ensuremath{\mathbb{T}^*}\xspace}

\newcommand{\dom}{\ensuremath{\mathit{dom}}}

%%%%%%%%%%% FROM ANOTHER PAPER ON Nested SRV

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%% Runtime Verification Macros
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\newcommand{\Clock}{\textit{clock}}
\newcommand{\Xclock}{\ensuremath{X_\Clock}}
\newcommand{\SRV}{SRV\xspace}
\newcommand{\NRV}{NestedSRV\xspace}

%%%% types
\newcommand{\BoolT}{\textit{Bool}}
\newcommand{\NatT}{\textit{Nat}}
\newcommand{\IntT}{\textit{Int}}
\newcommand{\StackT}{\textit{Stack}}
\newcommand{\SetT}{\textit{Set}}
\newcommand{\ElemT}{\textit{Elem}}
\newcommand{\andsym}{\texttt{and}}
\newcommand{\orsym}{\texttt{or}}
\newcommand{\notsym}{\texttt{not}}
\newcommand{\truesym}{\texttt{true}}
\newcommand{\falsesym}{\texttt{false}}
\newcommand{\SP}{\hspace{0.03em}}

\newcommand{\ifthenelsesym}{
  $\begin{bmatrix}
    \sym{if}\SP\cdot\SP\sym{then}\SP\cdot\SP\\
        \hspace{0.12em}\sym{else}\SP\cdot\SP
  \end{bmatrix}$}
\newcommand{\ifthenelsetype}[1]{
  $\begin{array}{l}\BoolT \times #1 \times #1\\
    \hspace{3em}\Into #1
  \end{array}$
}
\newcommand{\BoolName}{\textit{Booleans}}
\newcommand{\BoolSorts}{\BoolT}
\newcommand{\NatName}{\textit{Naturals}}
\newcommand{\NatSorts}{\NatT, \BoolT}
\newcommand{\SetName}{\textit{Sets}}
\newcommand{\SetSorts}{\SetT, \BoolT, \ElemT}
\newcommand{\StackName}{\textit{Stacks}}
\newcommand{\StackSorts}{\StackT, \BoolT, \ElemT}

%%%%%

\newcommand{\Sres}{S_{\text{res}}}
\newcommand{\calS}{\mathcal{S}}
\newcommand{\calF}{\mathcal{F}}
\newcommand{\NExpr}{\ensuremath{\textit{NestedExpr}}}
\newcommand{\NestedAtomic}[1]{\ensuremath{\textit{NestedOffset}(#1)}}
\newcommand{\Atomic}[1]{\ensuremath{\textit{Offset}(#1)}}
%\newcommand{\In}{\mathcal{I}}
%\newcommand{\Out}{\mathcal{O}}
\newcommand{\Dom}{\mathcal{D}}
%\newcommand{\sym}[1]{#1}
%\newcommand{\sym}[1]{\ensuremath{\mathtt{#1}}}
\newcommand{\sym}[1]{\ensuremath{\mathtt{#1}}}
\newcommand{\symIF}{\sym{if}}
\newcommand{\symTHEN}{\sym{then}\xspace}
\newcommand{\symELSE}{\sym{else}\xspace}
\newcommand{\symTRUE}{\sym{true}\xspace}
\newcommand{\symFALSE}{\sym{false}\xspace}
\newcommand{\symf}{\sym{f}}
%\newcommand{\DOM}[1]{{#1}^{\Dom}}
\newcommand{\domf}{\DOM{f}}
\newcommand{\clock}[1]{\ensuremath{\text{$#1$}}\xspace}
\newcommand{\clockn}{\clock{n}}
\newcommand{\symDIV}{\sym{div}}
\newcommand{\otau}{\overline{\tau}}
\newcommand{\osigma}{\overline{\sigma}}
\newcommand{\anext}[3]{\ensuremath{#1 \leadsto_{#3} #2}}


\newcommand{\Pred}{\ensuremath{\textit{pred}}}
% Language name
\newcommand{\NSRV}{NestedSRV\xspace}
\newcommand{\LOLA}{LOLA\xspace}


% Translation stuff
\newcommand{\tigger}{trigger\xspace}
\newcommand{\tiggers}{triggers\xspace}
\newcommand{\Tiggers}{Triggers\xspace}

% To change!!!
\newcommand{\SIC}{\ensuremath{\parallel_{\mathcal{P}}}}

\newcommand{\ctrue}{\tbf{true}}
\newcommand{\cfalse}{\tbf{false}}

%\newcommand{\default}{c}

% Specification
\newcommand{\Spec}{\varphi}

% Input variables
\newcommand{\iv}{t}
\newcommand{\ivcall}{\iv_{call}}
\newcommand{\ivbeg}{\iv_{beg}}
\newcommand{\ivend}{\iv_{end}}
\newcommand{\ivret}{\iv_{ret}}
% Output variable
\newcommand{\ov}{s}
% Any stream variable 
\newcommand{\asv}{v}


% Output stream
\newcommand{\os}{\sigma}
% Input streams
\newcommand{\is}{\tau}
\newcommand{\iscall}{\is_{call}}
\newcommand{\isbeg}{\is_{beg}}
\newcommand{\isend}{\is_{end}}
\newcommand{\isret}{\is_{ret}}
% Any stream
\newcommand{\as}{\sigma}

% Abstract sum over execution model
\newcommand{\asum}[1]{\oplus_{#1}}
\newcommand{\aminus}[1]{\ominus_{#1}}

% Guess
\newcommand{\G}{\mathcal{G}}

\newcommand{\gaprev}[1]{\ensuremath{#1 . \ttt{prev}_{abs}}}
\newcommand{\gcprev}[1]{\ensuremath{#1 . \ttt{prev}_{con}}}
\newcommand{\gnow}[1]{\ensuremath{#1 . \ttt{now}}}
\newcommand{\gcnext}[1]{\ensuremath{#1 . \ttt{next}_{con}}}
\newcommand{\ganext}[1]{\ensuremath{#1 . \ttt{next}_{abs}}}

% Input
\newcommand{\inp}{\sigma}
\newcommand{\Inp}{\Sigma}

% Execution model
\newcommand{\exm}{\eta}
\newcommand{\Exm}{H}

% Automata
\newcommand{\LA}[1]{\mathcal{L}(#1)}

% Path
\newcommand{\path}{\alpha}

% Common types
\newcommand{\FNat}{\Nat_\bot}

% Brackets, tuples
\newcommand{\Bracket}[1]{\llbracket #1 \rrbracket}
\newcommand{\Tup}[1]{\ensuremath{\langle #1 \rangle}}

% Felipe's notes
\newcommand{\felitodo}[1]{\todo[linecolor=red,backgroundcolor=red!25,bordercolor=red]{Felipe: #1}}
\newcommand{\felitext}[1]{\todo[inline,linecolor=red,backgroundcolor=red!25,bordercolor=red]{Felipe: #1}}


\definecolor{darkblue}{rgb} {0.200, 0.200, 0.800}
\definecolor{darkred} {rgb} {0.800, 0.200, 0.200}
\definecolor{darkgreen}{rgb}{0.200, 0.800, 0.200}

\newcommand{\colorEv}[2]{\ensuremath{\textcolor{#2}{\llbracket} #1
    \textcolor{#2}{\rrbracket}}}
\newcommand{\colorSigmaEval}[3]{\ensuremath{\colorEv{#1}{#3}_{#2}}}
\newcommand{\colorEval}[2]{\colorEv{#1}{#2}}
\newcommand{\colorEvalSigma}[2]{\colorSigmaEval{#1}{\sigma}{#2}}
%\newcommand{\evalSpec}[1]{\colorSigmaEval{#1}{darkblue}}
\newcommand{\evalSpec}[1]{\colorEval{#1}{black}}
\newcommand{\evalSpecsigma}[2]{\colorEval{#1}{#2}{black}}
\newcommand{\evalE}[1]{\colorEval{#1}{darkred}}
\newcommand{\evalEsigma}[2]{\colorSigmaEval{#1}{#2}{darkred}}
%\newcommand{\evalTau}[1]{\colorSigmaEval{#1}{darkgreen}}
\newcommand{\evalTau}[1]{\colorEvalSigma{#1}{darkblue}}
\newcommand{\evalTauN}[1]{\colorEval{#1}{darkblue}}
\newcommand{\evalTausigma}[2]{\colorSigmaEval{#1}{#2}{darkblue}}
\newcommand{\evalTicks}[1]{\colorEvalSigma{#1}{brown}}
\newcommand{\evalTicksN}[1]{\colorEval{#1}{brown}}
\newcommand{\evalTickssigma}[2]{\colorSigmaEval{#1}{#2}{brown}}
\newcommand{\presentLabel}{\ensuremath{\mathcal{O}}}
\newcommand{\pastLabel}{\ensuremath{\prec}}
\newcommand{\edgesSpec}{\ensuremath{Edges_\spec}}
\newcommand{\interp}{\mathcal{I}}
\newcommand{\Val}{\mathit{V}}

%\newcommand{\undef}{\reserved{undef}}

\newcommand{\specialbot}[2]{\ensuremath{\bot^{#1}_{\text{#2}}}\xspace}
\newcommand{\untypedspecialbot}[1]{\ensuremath{\bot_{\text{#1}}}\xspace}
\newcommand{\D}{D}

% \newcommand{\maybe}[2]{\ensuremath{\mathtt{Maybe}}^#1_{\text{#2}}}
\newcommand{\T}{\ensuremath{\mathbb{T}}\xspace}
\newcommand{\outT}{\specialbot{\T}{outside}}
\newcommand{\outD}{\specialbot{\D}{outside}}
\newcommand{\notickD}{\specialbot{\D}{notick}}
\newcommand{\outDS}{\Syntax{outside}_\D}
\newcommand{\outTS}{\Syntax{outside}_{\T}}
\newcommand{\notickDS}{\Syntax{notick}_\D}
\newcommand{\maybe}[2]{\ensuremath{#1 \cup \{\specialbot{#1}{#2}\}}}
% \newcommand{\outT}{\untypedspecialbot{outside}}
% \newcommand{\outD}{\untypedspecialbot{outside}}
% \newcommand{\notickD}{\untypedspecialbot{notick}}
% \newcommand{\outDS}{\Syntax{outside}}
% \newcommand{\outTS}{\Syntax{outside}}
% \newcommand{\notickDS}{\Syntax{notick}}

\newcommand{\maybeOutT}{\maybe{\T}{outside}}
\newcommand{\maybeOutD}{\maybe{D}{outside}}
\newcommand{\maybeNotickD}{\maybe{D}{notick}}
\newcommand{\undef}{\reserved{undef}} % Might be confusing with bottom

\newcommand{\entails}{\vdash}
\newcommand{\nonZenoT}{2^{\T}_{nz}}
\newcommand{\offsetEps}{\T_\epsilon}

\newcommand{\lambdatS}[1]{\Syntax{(\text{\textlambda} t . }#1\Syntax{)}}
\newcommand{\evalAlphaT}[1]{\colorSigmaEval{#1}{black}\alpha_t}
\newcommand{\evalAlpha}[1]{\colorSigmaEval{#1}{black}\alpha}

\newcommand{\Eval}{\mathit{Eval}\xspace}
\newcommand{\EvalPhi}{\ensuremath{\Eval_\varphi}\xspace}

% Processors
\newcommand{\colorboxnode}[2]{%
    \colorlet{currentcolor}{.}%
    {\color{#1}%
    \fbox{\color{currentcolor}\strut \ensuremath{#2}}}%
    \xspace
}
\newcommand*{\tickNode}[1]{\colorboxnode{green}{#1}}
\newcommand*{\valueNode}[1]{\colorboxnode{blue}{#1}}
\newcommand*{\gateNode}[1]{\colorboxnode{black}{#1}}

\newcommand*{\delayTickNode}{\tickNode{delay}}
\newcommand*{\srcTickNode}{\tickNode{srcTick}}
\newcommand*{\constTickNode}{\tickNode{constTick~c}}
\newcommand*{\UTickNode}{\tickNode{UTick}}

\newcommand*{\prevNode}{\valueNode{prev}}
\newcommand*{\prevEqNode}{\valueNode{prevEq}}
\newcommand*{\prevValNode}{\valueNode{prevVal}}
\newcommand*{\prevEqValNode}{\valueNode{prevEqVal}}
\newcommand*{\funcNode}{\valueNode{func~f}}
\newcommand*{\tNode}{\valueNode{\mathbf{t}}}

\newcommand*{\coreNode}{\gateNode{core}}
\newcommand*{\inputNode}{\gateNode{in}}

\newcommand*{\StreamT}[1]{\ensuremath{\mathcal{S}_{#1}}}
\newcommand*{\StreamProgressT}[1]{\ensuremath{\mathcal{S}^{\progressEv}_{#1}}}
\newcommand*{\StreamUnit}{\StreamT{Unit}}
\newcommand*{\StreamProgressUnit}{\StreamProgressT{Unit}}

% Processor functions
\newcommand*{\voteFun}{\ensuremath{vote}\xspace}
\newcommand*{\execFun}{\ensuremath{exec}\xspace}
\newcommand*{\rinseFun}{\ensuremath{rinse}\xspace}
\newcommand*{\mayTickFun}{\ensuremath{mayTick}\xspace}
\newcommand*{\computeValFun}{\ensuremath{computeVal}\xspace}

% Progress events data
\newcommand*{\progressEv}{\untypedspecialbot{progress}}

% Translation phase
\newcommand*{\signalFun}{\ensuremath{signalNode}\xspace}
\newcommand*{\translateTicks}[1]{\ensuremath{translateTicks(#1)}\xspace}
\newcommand*{\translateSpec}{\ensuremath{translateSpec}\xspace}
\newcommand*{\translateVal}[1]{\ensuremath{translateVal(#1)}\xspace}

% System state
\newcommand*{\quiescT}{\ensuremath{\T \cup \{-\infty\}}\xspace}
\newcommand*{\globalSystem}{\ensuremath{S}\xspace}
\newcommand*{\graph}{\ensuremath{G}\xspace}
\newcommand*{\graphT}{\ensuremath{\tupleof{V,E}}\xspace}
\newcommand*{\eStates}{\ensuremath{\Sigma_E}\xspace}
\newcommand*{\vStates}{\ensuremath{\Sigma_V}\xspace}
\newcommand*{\inputTagT}{\ensuremath{InTag}\xspace}
\newcommand*{\nodeStateT}{\ensuremath{nodeState}\xspace}
\newcommand*{\edgeStateT}{\ensuremath{edgeState}\xspace}
\newcommand*{\vStateFunT}{\ensuremath{(V \to \nodeStateT)}\xspace}
\newcommand*{\eStateFunT}{\ensuremath{(V \times \inputTagT \to \edgeStateT)}\xspace}
\newcommand*{\dynSys}{\ensuremath{\Sigma}\xspace}
\newcommand*{\dynSysT}{\ensuremath{\tupleof{\vStateFunT, \eStateFunT}}\xspace}
\newcommand*{\portTag}[1]{\ensuremath{\mathtt{#1}}\xspace}

% Channel functions
\newcommand*{\writeChansFun}{\ensuremath{writeChannels}\xspace}
\newcommand*{\readChansFun}{\ensuremath{readChannels}\xspace}
\newcommand{\emptyChannel}{\specialbot{\D}{emptychannel}}

% Operational semantics
\newcommand{\ticksDef}[1]{\mathcal{E}^{ticks}_{#1}}
\newcommand{\valsDef}[1]{\mathcal{E}^{vals}_{#1}}



\newcommand{\colorHEval}[2]{\colorSigmaEval{#1}{H}{#2}}
\newcommand{\evalEH}[1]{\colorHEval{#1}{darkred}}
\newcommand{\evalTicksH}[1]{\colorHEval{#1}{brown}}

\newcommand{\opEval}[5]{\colorSigmaEval{#4}{#5}{#2\vert_{#1,#3}}(#3)}
\newcommand{\mayTick}[4]{\opEval{#2}{#3}{#4}{#1}{brown}}
\newcommand{\computeVal}[4]{\opEval{#2}{#3}{#4}{#1}{darkred}}
\newcommand{\computeTau}[4]{\opEval{#2}{#3}{#4}{#1}{darkblue}}

% Dependency graph
\newcommand{\ddep}{\rightarrow}
\newcommand{\ddepPres}{\xrightarrow{0}}
\newcommand{\ddepPresStar}{\xrightarrow{\smash{0}}^*}

\newcommand{\ddepPast}{\xrightarrow{-}}
\newcommand{\ddepFut}{\xrightarrow{+}}

\newcommand{\Present}{\textit{Present}}
\newcommand{\Past}{\textit{Past}}
\newcommand{\Future}{\textit{Future}}

%%%% For algorithmic

% New definitions
\algnewcommand\algorithmicswitch{\textbf{switch}}
\algnewcommand\algorithmiccase{\textbf{case}}
\algnewcommand\algorithmicassert{\texttt{assert}}
\algnewcommand\Assert[1]{\State \algorithmicassert(#1)}%
% New "environments"
\algdef{SE}[SWITCH]{Switch}{EndSwitch}[1]{\algorithmicswitch\ #1\ \algorithmicdo}{\algorithmicend\ \algorithmicswitch}%
\algdef{SE}[CASE]{Case}{EndCase}[1]{\algorithmiccase\ #1}{\algorithmicend\ \algorithmiccase}%
\algtext*{EndSwitch}%
\algtext*{EndCase}%

%%%
\newcommand{\SUP}{\ensuremath{\mathit{sup}}}

\newcommand{\tin}{\ensuremath{t_\textit{in}}}
%\newcommand{\tqin}{\ensuremath{t_q^{\textit{in}}}}
\newcommand{\tqin}{\tin}
\newcommand{\tout}{\ensuremath{t_\textit{out}}}
%\newcommand{\tqout}{\ensuremath{t_q^{\textit{out}}}}
\newcommand{\tqout}{\tout}
\newcommand{\append}{\textit{append}}
\newcommand{\tq}{\ensuremath{t_q}}

\newcommand{\App}{\ensuremath{\mathrel{\scalebox{0.8}{++}}}}

\newcommand{\PrevStt}[1]{\ensuremath{\textbf{\texttt{<<}}~#1}}
\newcommand{\PrevEqStt}[1]{\ensuremath{\textbf{\texttt{<\~}}~#1}}

\newcommand{\SY}[1]{\text{\texttt{#1}}}
\newcommand{\PrevEqV}[1]{\SY{(\~}#1\SY{)}}
\newcommand{\PrevV}[1]{\SY{(<}#1\SY{)}}
\newcommand{\SuccEqV}[1]{\SY{(}#1\SY{~)}}
\newcommand{\SuccV}[1]{\SY{(}#1\SY{>)}}


==> figures/latex/macros/altba.tex <==
\newcommand{\var}{{\mathcal{X}}}
\newcommand{\posform}[1]{\mathcal{B}^+(#1)}

%%% Local Variables: 
%%% mode: latex
%%% TeX-master: "../main"
%%% End: 


==> figures/latex/macros/automata.tex <==
%\newcommand{\AutNode}[1]{*+[F-:<3pt>]{#1}}
\newcommand{\AutNode}[1]{*+[o][F-]{#1}}
\newcommand{\AutFinalNode}[1]{*+[o][F=]{#1}}

==> figures/latex/macros/colors.tex <==
\newcommand{\VLC}[1]{\textcolor{darkgreen}{#1}}
\newcommand{\VRC}[1]{\textcolor{darkred}{#1}}
\newcommand{\emphC}[1]{\textcolor{red}{#1}}
\newcommand{\GR}[1]{\textcolor{darkgreen}{#1}}
\newcommand{\RD}[1]{\textcolor{darkred}{#1}}
\newcommand{\BL}[1]{\textcolor{darkblue}{#1}}
\newcommand{\ORN}[1]{\textcolor{darkorange}{#1}}
\newcommand{\ColRE}[1]{\ORN{#1}}
\newcommand{\ColTL}[1]{\RD{#1}}
\newcommand{\ColAUT}[1]{\BL{#1}}
\newcommand{\ColL}[1]{\GR{#1}}

\newcommand{\Cr}{\ColRE{r}}
\newcommand{\Cs}{\ColRE{s}}
\newcommand{\Cx}{\ColTL{x}}
\newcommand{\Cy}{\ColTL{y}}
\newcommand{\Cz}{\ColTL{z}}
\newcommand{\spc}{\hspace{2em}}
\newcommand{\one}{\ColRE{\textit{one}}}
\newcommand{\mwm}{\ColRE{\textit{mwm}}}
\newcommand{\wm}{\ColRE{\textit{wm}}}
\newcommand{\mr}{\ColRE{\textit{mr}}}
\newcommand{\ttrue}{\ColTL{\texttt{true}}}
\newcommand{\Henceforth}{\ColTL{\textbf{G}}}
\newcommand{\ABS}{\ColRE{\textit{abs}}}
\newcommand{\CALLER}{\ColRE{\textit{caller}}}
\newcommand{\sumOne}{\ColRE{\textit{sum1}}}
\newcommand{\sumTwo}{\ColRE{\textit{sum2}}}
\newcommand{\Aut}[1]{\ensuremath{\mathcal{#1}}}
\newcommand{\AutA}{\Aut{A}}


==> figures/latex/macros/direct.tex <==
\newcommand{\Direct}{\textsc{Direct}\xspace}
\newcommand{\into}{\rightarrow}

%%%% FIGURE WITH 2 PROGRAMS
\begin{SaveVerbatim}[fontfamily=courier]{Thread-1}
1  void infa(void)  {
2    while (1) {
3      if (exp) {
4        mutex_lock(b);
5        mutex_lock(a);
6        // critical sect
7        mutex_unlock(a);
8        mutex_unlock(b);
9     } else {
10       mutex_lock(c);
11       mutex_lock(a);
12       // critical sect
13       mutex_unlock(a);
14       mutex_unlock(c);
15     }
16   }
17 }
\end{SaveVerbatim}

\begin{SaveVerbatim}[fontfamily=courier]{Thread-2}
21 void infb(void) {
22   while (1) {
23     mutex_lock(a);
24     mutex_lock(b);
25     // critical sect
26     mutex_unlock(b);
27     mutex_unlock(a);
28   }
29 }
\end{SaveVerbatim}

%%%%% TRACE OF DINING PHILOSPHERS
\newcommand{\DiningTrace}{
\begin{tabular}{|l||l|l|l|l|l|l|l|l|l|}
        \hline
$\textit{State}$ & $\textit{Thrd}$ & 
\multicolumn{5}{|c|}{\textit{Philosopher threads}} & \textit{Res} & \textit{Res} & $\textit{(c)alls/}$ \\
$\textit{no.}$ & $\textit{id}$ & $T_0$ & $T_1$ & $T_2$ & $T_3$ & $T_4$ & $\textit{values}$ & $\textit{held}$ & $\textit{(r)ets}$ \\
        \hline \hline
$1$  & $3$ &  $(0, 2)$ &  $(0, 2)$ &  $(0, 2)$ &  $(0, 1)$ &  $(0, 0)$ & $(0,0,0,1,1)$ & $()$ & $c$ \\
\rowcolor[rgb]{0.90,0.99,0.90}$2$  & $3$ &  $(0, 2)$ &  $(0, 2)$ &  $(0, 2)$ &  $(0, 1)$ &  $(0, 0)$ & $(0,0,0,0,1)$ & $(3)$ & $r$ \\
$3$  & $3$ &  $(0, 2)$ &  $(0, 2)$ &  $(0, 2)$ &  $(0, 2)$ &  $(0, 0)$ & $(0,0,0,0,1)$ & $(3)$ & $c$ \\
$4$  & $4$ &  $(0, 2)$ &  $(0, 2)$ &  $(0, 2)$ &  $(0, 2)$ &  $(0, 0)$ & $(0,0,0,0,1)$ & $()$ & $r$ \\
\rowcolor[rgb]{0.99,0.90,0.90}$5$  & $4$ &  $(0, 2)$ &  $(0, 2)$ &  $(0, 2)$ &  $(0, 2)$ &  $(0, 1)$ & $(0,0,0,0,1)$ & $()$ & $c$ \\
\rowcolor[rgb]{0.99,0.80,0.80}$6$  & $4$ &  $(0, 2)$ &  $(0, 2)$ &  $(0, 2)$ &  $(0, 2)$ &  $(0, 1)$ & $(0,0,0,0,0)$ & $(4)$ & $r$ \\
$\ldots$  & $\ldots$ &  &  &  &  &  & & & \\
$16$ & $4$ &  $(0, 3)$ &  $(0, 3)$ &  $(0, 3)$ &  $(0, 3)$ &  $(0, 2)$ & $(0,0,0,0,0)$ & $(4)$ & $r$ \\
\rowcolor[rgb]{0.90,0.70,0.70}$17$ & $4$ &  $(0, 3)$ &  $(0, 3)$ &  $(0, 3)$ &  $(0, 3)$ &  $(0, 3)$ & $(0,0,0,0,0)$ & $(4)$ & $c$ \\
        \hline
\end{tabular}
}



==> figures/latex/macros/enriched.tex <==
%%%%% %%%%% 1. for the enriched paper %%%%%
%\newcommand{\F}{\mathsf{F}} %\newcommand{\T}{\mathsf{T}}
%\newcommand{\F}{\mathbf{false}}
%\newcommand{\T}{\mathbf{true}}
%\newcommand{\true}{\T}
%\providecommand*{\Always}{} %Ale: to compile with cesar-llncs
%\renewcommand{\Always}{\LTLsquare}
%\providecommand*{\Event}{} %Ale: to compile with cesar-llncs
%\renewcommand{\Event}{\LTLdiamond}
%\providecommand*{\Next}{} %Ale: to compile with cesar-llncs
%\renewcommand{\Next}{\LTLcircle}
%\newcommand{\Prev}{\LTLcircleminus}
%\newcommand{\PrevNoFirst}{\LTLcircletilde}
%\newcommand{\HasAlwaysBeen}{\LTLsquareminus}
%\providecommand*{\Once}{} %Ale: to compile with cesar-llncs
%\renewcommand{\Once}{\LTLdiamondminus}
%\providecommand*{\Since}{} %Ale: to compile with cesar-llncs
%\renewcommand{\Since}{\mathbin{\mathcal{S}}}
%\providecommand*{\BackTo}{} %Ale: to compile with cesar-llncs
%\renewcommand{\BackTo}{\mathbin{\mathcal{B}}}
%\newcommand{\WeakPrev}{\LTLcircletilde}


\newcommand{\ORsym}{{\scriptstyle{\pmb{+}}}}
\newcommand{\SEQsym}{{\scriptstyle{\cdot}}}
\newcommand{\ANDsym}{{\scriptstyle{\pmb{|}}}}
\newcommand{\STARsym}{*}
\newcommand{\EXPsym}{\widehat{\;\phantom{\cdot}\;}}
\newcommand{\POWsym}{\EXPsym}
\newcommand{\DPOWsym}{\_}
\newcommand{\NEGsym}{\overline{\;\phantom{\cdot}\;}}
%\newcommand{\INF}[1]{\overset{\infty}{#1}}
\newcommand{\INF}[1]{\widehat{#1}}
%\newcommand{\ORsymInf}{\INF{\ORsym}}
\newcommand{\ORsymInf}{\oplus}
%\newcommand{\ANDsymInf}{\INF{\ANDsym}}
\newcommand{\ANDsymInf}{\oslash}
%\newcommand{\SEQsymInf}{\INF{\SEQsym}} 
\newcommand{\SEQsymInf}{\odot} 
\newcommand{\OR}{\mathrel{+}}
\newcommand{\AND}{\mathrel{|}} 
\newcommand{\SEQ}{\mathrel{\cdot}}
%\newcommand{\ORInf}{\mathrel{\INF{\scriptstyle{+}}}}
\newcommand{\ORInf}{\mathrel{\oplus}}
%\newcommand{\ANDInf}{\mathrel{\INF{\scriptstyle{|}}}}
\newcommand{\ANDInf}{\mathrel{\oslash}}
%\newcommand{\SEQInf}{\mathrel{\INF{\scriptstyle{\cdot}}}}
\newcommand{\SEQInf}{\mathrel{\odot}}

\newcommand{\uSTAR}{^\STARsym} %unary star
\newcommand{\bSTAR}{\mathrel{\STARsym}} %unary star
\newcommand{\STAR}{\uSTAR} \newcommand{\CIRC}{\mathrel{\circ}}
%\newcommand{\EnrichedRE}{E$\omega${}RE\xspace}
\newcommand{\EnrichedRE}{\ensuremath{\textup{EnRE}}\xspace}
\newcommand{\EnRE}{\EnrichedRE}
\newcommand{\VeryEnrichedRE}{kE$\omega${}RE\xspace}
%\newcommand{\Vars}{\mathcal{V}}
\newcommand{\ElemRE}{\ensuremath{\textup{ElemRE}}\xspace}
%\newcommand{\Bool}{\mathcal{B}}
\newcommand{\wRE}[1]{\ensuremath{\omega\text{RE}(#1)}}
\newcommand{\finRE}[1]{\ensuremath{\text{RE}(#1)}}
\newcommand{\RE}{\textup{RE}\xspace} % regular expressions
\newcommand{\ERE}{\textup{ERE}\xspace} % Extended Regular Expressions RE(+,*,;,|,~,[w]) 
\newcommand{\SERE}{\textup{SERE}\xspace} %Semi-Extended Regular Expressions RE(+,*,;,|, ,[w])

\newcommand{\SigmaElem}{\Sigma_\text{elem}}
\newcommand{\SigmaEnriched}{\Sigma_\text{rich}}
\newcommand{\SigmaEnrichedInf}{\Sigma^{\omega}_\text{rich}}
\newcommand{\SigmaRegexp}{\Sigma_\text{regexp}}

\newcommand{\NBW}{NBW\xspace} % non-deterministic B\"uchi automata on words 
\newcommand{\DBW}{DBW\xspace} % deterministic B\"uchi automata on words 
\newcommand{\ABW}{ABW\xspace} % alternating B\"uchi automata on words 
\newcommand{\BABW}{BABW\xspace} %
\newcommand{\ETL}{\text{ETL}\xspace} % Extended Temporal Logic ETL
\newcommand{\ETLr}{\ensuremath{\text{ETL}_r}\xspace} % ETL (regular condition) 
\newcommand{\ETLl}{\ensuremath{\text{ETL}_l\xspace}} % ETL (loop condition) 
\newcommand{\ETLf}{\ensuremath{\text{ETL}_f\xspace}}
% ETL (finite condition)
\newcommand{\ETLa}{\ensuremath{\text{ETL}_a\xspace}} % ETL(alternating condition)
\newcommand{\ETLta}{\ensuremath{\text{ETL}_2a}\xspace} % ETL (two way alternating condition) 
\newcommand{\Release}{\mathbin{\mathcal{R}}}

\newcommand{\ALL}{\ensuremath{\mathbf{all}}\xspace}

%\newcommand{\Alphabet}{\Gamma}
\newcommand{\Alphabet}{\Sigma}

\newcommand{\Eqs}{\mathcal{E}}


\newcommand{\DefOR}{\ensuremath{\;\;\;\big|\;\;\;}}
\renewcommand{\SEQsym}{\ensuremath{;}}
\renewcommand{\SEQ}{\mathrel{\SEQsym}}

\newcommand{\REOR}{+}
\newcommand{\RESEQsym}{\ensuremath{;}}
\newcommand{\RESeq}{\mathrel{\RESEQsym}}
\newcommand{\REStar}{*}


==> figures/latex/macros/general.tex <==
\newcommand\Def[2][]{%                        % F"ur Definitionen 
  \def\temp{#1}%                              % die in den Index sollen
  \ifx\temp\empty%
    \def\temp{#2}%
  \fi%
%{\em\boldmath#2\unboldmath\index{\temp}}}
{\em#2\index{\temp}}}

\newcommand{\N}{\mathbb{N}}

\newcommand{\onlyWithComplement}[1]{}

%\newcommand{\pos}{\textit{pos}}
%\newcommand{\Pos}{\textit{Pos}}
\newcommand{\pos}{\omega}
\newcommand{\Pos}{\omega}



%%% Local Variables: 
%%% mode: latex
%%% TeX-master: "../main"
%%% End: 


==> figures/latex/macros/macros.tex <==
\input{macros/general}
\input{macros/enriched}
\input{macros/rules}
\input{macros/altba}
\input{macros/automata}
\input{macros/direct}
\input{macros/colors}

==> figures/latex/macros/rules.tex <==

%\newcommand{\AccSym}{\uparrow}
% \newcommand{\AccSym}{\tick}
%%\RequirePackage{pifont}
%% \newcommand{\tick}{\ding{51}}
%% \newcommand{\AccSym}{\tick}

\RequirePackage{amssymb}
\newcommand{\AccSym}{\surd}


%\newcommand{\RejSym}{\downarrow}
\RequirePackage{pifont}
%\newcommand{\RejSym}{\text{\ding{53}}}
\newcommand{\RejSym}{\,\mathsf{x}\,}

% \newcommand{\ACC}[1]{\ensuremath{\overset{#1}{\AccSym}}}
 \newcommand{\ACC}[1]{\ensuremath{{\AccSym}\hspace{-0.7em}{\overset{#1}{\text{\phantom{x}}}}}}
 \newcommand{\ACCa}{\ACC{s}}
 \newcommand{\REJ}[1]{\ensuremath{\overset{#1}{\RejSym}}}
 \newcommand{\REJa}{\REJ{s}}
 \newcommand{\DER}[1]{\ensuremath{\overset{#1}{\Into}}}
 \newcommand{\DERa}{\DER{s}}

 \newcommand{\BasicAcceptRuleA}{\ell \ACCa\;\;\text{(if $s\models \ell$)}}
 \newcommand{\BasicAcceptRuleB}{\ell \REJa\;\;\text{(if $s\nmodels \ell$)}}
 \newcommand{\BasicNextRule}{\ell \DERa \F}


 \newcommand{\ORAcceptRuleA}{
   \AxiomC{$x\ACCa$}
   %\LeftLabel{\ORAcceptRuleALabel}
   \UnaryInfC{$x \OR y \ACCa$}
   \DisplayProof
 }
 \newcommand{\ORAcceptRuleB}{
   \AxiomC{$y\ACCa$}
   %\LeftLabel{\ORAcceptRuleALabel}
   \UnaryInfC{$x \OR y \ACCa$}
   \DisplayProof
 }
 \newcommand{\ORAcceptRuleC}{
      \AxiomC{$x\REJa$}
      \AxiomC{$y\REJa$}
      %\LeftLabel{\ORAcceptRuleALabel}
      \BinaryInfC{$x \OR y \REJa$}
      \DisplayProof
 }
 \newcommand{\OrNextRule}{
      \AxiomC{$x\DERa x'$}
      \AxiomC{$y\DERa y'$}
      %\LeftLabel{\ORAcceptRuleALabel}
      \BinaryInfC{$x \OR y \DERa x' \OR y'$}
      \DisplayProof
 }

 \newcommand{\AndAcceptRuleA}{
   \AxiomC{$x\REJa$}
   %\LeftLabel{\ORAcceptRuleALabel}
   \UnaryInfC{$x \AND y \REJa$}
   \DisplayProof
   
 }
 \newcommand{\AndAcceptRuleB}{
   \AxiomC{$y\REJa$}
   %\LeftLabel{\ORAcceptRuleALabel}
   \UnaryInfC{$x \AND y \REJa$}
   \DisplayProof
}
\newcommand{\AndAcceptRuleC}{
  \AxiomC{$x\ACCa$}
  \AxiomC{$y\ACCa$}
  %\LeftLabel{\ORAcceptRuleALabel}
  \BinaryInfC{$x \AND y \ACCa$}
  \DisplayProof
}
\newcommand{\AndNextRule}{
  \AxiomC{$x\DERa x'$}
  \AxiomC{$y\DERa y'$}
  %\LeftLabel{\ORAcceptRuleALabel}
  \BinaryInfC{$x \AND y \DERa x' \AND y'$}
  \DisplayProof
}

\newcommand{\SeqAcceptRule}{
  x \SEQ y \REJa
}

\newcommand{\SeqNextRuleA}{
  \AxiomC{$x\ACCa$}
  \AxiomC{$x\DERa x'$}
  %\LeftLabel{\ORAcceptRuleALabel}
  \BinaryInfC{$x \SEQ y \DERa x'\SEQ y \OR y$}
  \DisplayProof
}
\newcommand{\SeqNextRuleB}{
  \AxiomC{$x\REJa$}
  \AxiomC{$x\DERa x'$}
  %\LeftLabel{\ORAcceptRuleALabel}
  \BinaryInfC{$x \SEQ y \DERa x'\SEQ y$}
  \DisplayProof
}

\newcommand{\PowAcceptRuleA}{
  \AxiomC{$y\ACCa$}
  \UnaryInfC{$x^z y \ACCa$}
  \DisplayProof
}
\newcommand{\PowAcceptRuleB}{
  \AxiomC{$y\REJa$}
  \UnaryInfC{$x^z y \REJa$}
  \DisplayProof
}
\newcommand{\PowNextRuleA}{
  \AxiomC{$x\DERa x'$}
  \AxiomC{$y\DERa y'$}
  \AxiomC{$z\DERa z'\;\;\;\;z\REJa$}
  \TrinaryInfC{$x^z y \DERa y' \OR (x' \AND (z' \SEQ x^z y))\text{\phantom{$\OR x^z y$}}$}
  \DisplayProof
}
\newcommand{\PowNextRuleB}{
  \AxiomC{$x\DERa x'$}
  \AxiomC{$y\DERa y'$}
  \AxiomC{$z\DERa z'\;\;\;\;z\ACCa$}
  \TrinaryInfC{$x^z y \DERa y' \OR (x' \AND (z' \SEQ x^z y \OR x^z y))$}
  \DisplayProof
}

\newcommand{\DualPowAcceptRuleA}{
  \AxiomC{$y\REJa$}
  \UnaryInfC{$x_z y \REJa$}
  \DisplayProof
}
\newcommand{\DualPowAcceptRuleB}{
  \AxiomC{$y\ACCa$}
  \AxiomC{$x\ACCa$}
  \BinaryInfC{$x_z y \ACCa$}
  \DisplayProof
}
\newcommand{\DualPowAcceptRuleC}{
  \AxiomC{$y\ACCa$}
  \AxiomC{$x\REJa$}
  \BinaryInfC{$x_z y \REJa$}
  \DisplayProof
}



\newcommand{\DualPowNextRuleA}{
  \AxiomC{$x\DERa x'$}
  \AxiomC{$y\DERa y'$}
  \AxiomC{$z\DERa z'\;\;\;\;z\REJa$}
  \TrinaryInfC{$x_z y \DERa y' \AND (x' \OR (z' \SEQ x_z y))\text{\phantom{$\OR x^z y$}}$}
  \DisplayProof
}
\newcommand{\DualPowNextRuleB}{
  \AxiomC{$x\DERa x'$}
  \AxiomC{$y\DERa y'$}
  \AxiomC{$z\DERa z'\;\;\;\;z\ACCa$}
  \TrinaryInfC{$x_z y \DERa y' \AND (x' \OR (z' \SEQ x_z y \OR x_z y))$}
  \DisplayProof
}

\newcommand{\EquationAcceptRuleA}{
  \AxiomC{$\phi(x_1,\ldots) \ACCa$}
  \UnaryInfC{$\phi(x_1,\ldots) \ACCa_\Eqs$}
  \DisplayProof 
}

\newcommand{\EquationAcceptRuleB}{
  \AxiomC{$\phi(x_1,\ldots) \REJa$}
  \UnaryInfC{$\phi(x_1,\ldots) \REJa_\Eqs$}
  \DisplayProof 
}

\newcommand{\EquationNextRule}{ 
  \AxiomC{$\phi(x_1,\ldots,x_n) \DERa \phi'(x_1,\ldots,x_n)$} 
  \UnaryInfC{$\phi \DERa_\Eqs
    \phi'(\phi_{x_1},\ldots,\phi_{x_n})$} 
  \DisplayProof 
}


==> figures/latex/preamble.tex <==
\pdfobjcompresslevel0
\usepackage{fancyvrb}
\usepackage{amssymb}
\usepackage{amsmath}
\usepackage{algorithm}
\usepackage{algpseudocode}
\usepackage{cesar-llncs}
\input{theories}
\usepackage{xspace}
\usepackage{amssymb}
%\input{vpl-macros}
\input{macros}
\input{slidesaux}
\usepackage{mathtools}
\usepackage[ligature,reserved]{semantic}
\input{solidity-highlighting.tex}
\usepackage{paralist}
\usepackage{multicol}

\newcommand{\Hspeed}{H1}
\newcommand{\Hbetteralg}{H2}
\newcommand{\Hagr}{H3}
\newcommand{\Hbyzantine}{H4}
\newcommand{\Hdegrade}{H5}

\algblockdefx[Upon]{Upon}{EndUpon}%
[1]{{\bf upon} (#1) {\bf do}}%
{{\bf end upon}}
\algblockdefx[When]{When}{EndWhen}%
[1]{{\bf when} (#1) {\bf do}}%
{{\bf end when}}
\mathlig{<-}{\leftarrow}
\mathlig{==}{\equiv}
\mathlig{<<}{\langle}
\mathlig{>>}{\rangle}
%% Variables in implementation
\reservestyle{\variables}{\text}
\variables{epoch,current,history,theset[the\_set],pending, tobroadcast[to\_broadcast]}

\reservestyle{\setops}{\text}
\setops{add,get,Init,Add,Get,BAdd,EpochInc,Broadcast,Deliver,GetEpoch,Propose,SetDeliver}

\reservestyle{\structs}{\text}
\structs{DPO,BAB,BRB,SBC,DSO}

\reservestyle{\stmt}{\textbf}
\stmt{call,ack,drop,return,assert,wait}

\reservestyle{\messages}{\texttt}
\messages{madd[add],mepochinc[epinc]}

\reservestyle{\api}{\texttt}
\api{apiBAdd,apiAdd,apiGet,apiEpochInc,apiTheSet[{the\_set}],apiHistory}

\reservestyle{\schain}{\texttt}
\schain{history,epoch,theset[{the\_set}],add,get,epochinc[{epoch\_inc}],getepoch[{get\_epoch}],
Fast, Slow, Basic, Central}

\newcommand{\Servers}{N}

\usepackage{color, colortbl}

 \usepackage{tikz-timing}
 \usetikzlibrary{matrix, shapes.misc, decorations, decorations.pathreplacing, automata, fit}
 \tikzset{
 	ampersand replacement=\&, % alternative to using fragile frames
 	event/.style = {draw, cross out, inner sep = 1pt,xshift=0.75pt},
 	event label/.style = {font = \tiny, label distance = -2pt}  
 }

\usepackage{listings}
%% \lstset{
%% 	%  extendedchars=true,
%% 	%  inputencoding=utf8
%% 	basicstyle=\small\ttfamily,
%% 	%  stringstyle=
%% 	%  keywordsyle={[2]\underbar},
%% 	commentstyle=\rmfamily\it,
%% 	extendedchars=true,
%% 	keepspaces=true, 
%% 	columns=flexible,
%% %	frame=tlrb,
%% 	keywordstyle=\ttfamily\bfseries
%% }
\lstdefinestyle{long}{}
\lstdefinestyle{inline}{   
	basicstyle=\ttfamily\footnotesize,
	numbers=none,
	xleftmargin=2em,
	aboveskip=0.3ex,
	belowskip=0ex,
	%  belowcaptionskip=0em,
	%  lineskip=0em
}
\lstdefinelanguage{tessla}{
	keywords={on, if, fun, define, yield, out, trigger, while, window, and, in},
	keywordstyle=\ttfamily\color{darkblue}\bfseries,
	classoffset=1,
	morekeywords={EStream,VStream,Int,Bool},  
	%  keywordstyle=\ttfamily\bfseries,
	keywordstyle=\underline,
	classoffset=0,
	comment=[l]{--}
}
\definecolor{StriverBlue}{RGB}{42, 0, 255}
\definecolor{StriverGreen}{RGB}{0, 155, 0}
\definecolor{StriverRed}{RGB}{155, 0, 0}
\definecolor{StriverOrange}{RGB}{255, 183, 68}
\definecolor{StriverYellow}{RGB}{155, 155, 45}
\lstdefinelanguage{Striver}
{
    basicstyle=\ttfamily,
    keywordstyle=[1]\color{StriverYellow},
    keywordstyle=[2]\color{StriverBlue},
    keywordstyle=[3]\bfseries,
%    keywordstyle=[4]\itshape,
    keywordstyle=[4]\color{StriverBlue},
    keywordstyle=[5]\color{StriverOrange},
    keywordstyle=[6]\color{StriverGreen},
    keywordstyle=[7]\color{StriverRed},
%    otherkeywords = {
%    <~,<<,~>,>>,shift,macro,:=,const,input,output,true,false,ticks,define,outside,notick,U,delay,at,||,&&,+,-,==,!,!=,if,let,in then,else,char,int,bool,unit,Time,_eps,void},
    otherkeywords = {
    <~,<<,~>,>>,:=||,&&,+,-,==,!,!=},
    morekeywords = [1]{<~,<<,~>,>>},
    morekeywords = [2]{shift,macro, :=, input,const, output, ticks, define},
    morekeywords = [3]{outside, notick, true, false},
    morekeywords = [4]{if, then, else},
    morekeywords = [5]{char, int, bool, unit, Time, _eps, void},
    morekeywords = [6]{U, delay, ||, &&, +, -, !, !=, ==, at},
    morekeywords = [7]{let, in},
}
\lstdefinestyle{pseudo}{language={},%
 % basicstyle=\normalfont,%
 % keywordstyle=\normalfont\bfseries,%
  morecomment=[l]{//},%
  morekeywords={for,to,while,do,if,then,else,and,or,not},%
  mathescape=true,%
  columns=fullflexible
}


==> figures/latex/programs.tex <==
\newcommand{\RefFigListClass}{\ref{fig:programs}(a)\xspace}
\newcommand{\RefFigMGC}      {\ref{fig:programs}(b)\xspace}
\newcommand{\RefFigSearch}   {\ref{fig:programs}(c)\xspace}
\newcommand{\RefFigLocate}   {\ref{fig:programs}(d)\xspace}
\newcommand{\RefFigAdd}      {\ref{fig:programs}(e)\xspace}
\newcommand{\RefFigRemove}   {\ref{fig:programs}(f)\xspace}

\newcommand{\RefFigListClassGhost}{\ref{fig:programs:ghost}(a)\xspace}
\newcommand{\RefFigLocateGhost}		{\ref{fig:programs:ghost}(b)\xspace}
\newcommand{\RefFigAddGhost}			{\ref{fig:programs:ghost}(c)\xspace}
\newcommand{\RefFigRemoveGhost}		{\ref{fig:programs:ghost}(d)\xspace}

\newcommand{\FigLabel}[1]{\multicolumn{1}{c}{#1}}
\newcommand{\FigLabelWide}[1]{\multicolumn{3}{c}{#1}}

%
% Figures for data structure
%

\begin{SaveVerbatim}{list-data}
class List {
     Node list;
}
\end{SaveVerbatim}

\begin{SaveVerbatim}{list-data-space}
class List {
     Node list;

}
\end{SaveVerbatim}


\begin{SaveVerbatim}{node-data}
class Node {
     Value val;
     Node next;
     Lock lock;
}
\end{SaveVerbatim}

\newcommand{\DataStructuresBody}{
  \begin{tabular}{l}
    \renewcommand{\arraystretch}{0.4}
    $\begin{array}{l}
      \class \: \List \: \{ \\
      \mhs \Node \: \tList ;\\
      \}
    \end{array}$ \\ \\ \\
    \renewcommand{\arraystretch}{0.4}
    $\begin{array}{l}
      \class \: \Node \: \{ \\
      \mhs \Value \: \val ;\\
      \mhs \Node \: \tNext ;\\
      \mhs \Lock \: \lock ;\\
      \}
    \end{array}$
  \end{tabular}
}
\newcommand{\DataStructuresFig}{
\begin{minipage}[c]{3.7cm}
  \DataStructuresBody
\label{fig:listclass}
\end{minipage}
}

%
% Figures for most generate cliente "decide"
%
\newcommand{\MGCBody}{
  \begin{algorithmic}[1]
    \While {$\true$}
    \State $e := \NondetChooseElem$
    \State $\Nondet$
    \State $\left[ \begin{array}{l}
	\Call \search(e) \\
	\ProgOr \\
	\Call \add(e) \\
	\ProgOr \\
	\Call \remove(e)
      \end{array} \right]$
    \EndWhile
  \end{algorithmic}
}

\begin{SaveVerbatim}[fontfamily=courier]{mgc-prg}
0:  while true
1:     e:= NonDet();
2:     select
3:        search(e);
4:     or
5:        add(e);
6:     or
7:        remove(e);
8:  end;
\end{SaveVerbatim}

\newcommand{\MGCPrg}{
  \begin{minipage}[c]{5.0cm}
    \MGCBody
  \end{minipage}
}
\newcommand{\MGCFig}{
  \begin{minipage}[c]{4.1cm}
    \MGCBody
    \label{fig:mgc}
  \end{minipage}
}

%
% Figure for "search" 
%
\begin{SaveVerbatim}{search-prog}
20:  prev, cur := locate (e);
21:  if curr.val = e then
22:      result := true;
23:  else
24:      result := false;
25:  curr.unlock();
26:  prev.unlock();
27:  return result;
\end{SaveVerbatim}

\newcommand{\SearchBody}{
  \begin{algorithmic}[1]
    \State $\prev, \curr := \locate(e)$
    \If {$\curr.\val = e$}
    \State $\result := \true$
    \Else
    \State $\result := \false$
    \EndIf
    \State $\curr.\unlock()$
    \State $\prev.\unlock()$
    \State \tbf{return} $\result$
  \end{algorithmic}
}
\newcommand{\SearchPrg}{
  \begin{minipage}[c]{3.9cm}
    \SearchBody
  \end{minipage}
}
\newcommand{\SearchFig}{
\begin{minipage}[c]{3.9cm}
  \SearchBody
\label{fig:search}
\end{minipage}
}

%
% Figure for "locate"
%
\begin{SaveVerbatim}{locate-prog}
 9:  prev := Head;
10:  prev.lock();
11:  curr := prev.next;
12:  curr.lock();
13:  while curr.val < e do
14:      prev.unlock();
15:      prev := curr;
16:      curr := curr.next;
17:      curr.lock();
18:  end;
19:  return (prev,curr)
\end{SaveVerbatim}

\newcommand{\LocateBody}{
\begin{algorithmic}[1]
\State $\prev := \Head$
\State $\prev.\lock()$
\State $\curr := \prev.\tNext$
\State $\curr.lock()$
\While {$\curr.\val < e$}
	\State $\prev.\unlock()$
	\State $\prev := \curr$
	\State $\curr := \curr.\tNext$
	\State $\curr.\lock()$
\EndWhile
\State \tbf{return} $(\prev, \curr)$
\Statex
\end{algorithmic}
}

\newcommand{\LocatePrg}{
  \begin{minipage}[c]{3.7cm}
    \LocateBody
  \end{minipage}
}

\newcommand{\LocateFig}{
\begin{minipage}[c]{3.7cm}
  \LocateBody
\label{fig:locate}
\end{minipage}
}

%
% Figure for "add"
%
\begin{SaveVerbatim}{add-prog}
28:  prev, curr := locate(e);
29:  if curr.val != e then
30:      aux := new Node(e);
31:      aux.next := curr;
32:      prev.next := aux;
33:      result := true;
34:  else
35:      result := false;
36:  end;
37:  prev.unlock();
38:  curr.unlock();
39:  return result;
\end{SaveVerbatim}



\newcommand{\AddBody}{
\begin{algorithmic}[1]
\State $\prev, \curr := \locate(e)$
\If {$\curr.\val \neq e$}
	\State $\aux := \New \Node(e)$
	\State $\aux.\tNext := \curr$
	\State $\prev.\tNext := \aux$
	\State $\result := \true$
\Else
	\State $\result := \false$
\EndIf
\State $\prev.\unlock()$
\State $\curr.\unlock()$
\State \tbf{return} $\result$
\end{algorithmic}
}

\newcommand{\AddPrg}{
  \begin{minipage}[c]{4.1cm}
    \AddBody
  \end{minipage}
}

\newcommand{\AddFig}{
\begin{minipage}[c]{4.1cm}
  \AddBody
  \label{fig:add}
\end{minipage}
}

%
% Figure for "remove"
%
\begin{SaveVerbatim}{remove-prog}
40:  prev, curr := locate(e);
41:  if curr.val == e then
42:      aux := curr.next;
43:      prev.next := aux;
44:      result := true;
45:  else
46:      result := false;
47:  end;
48:  prev.unlock();
49:  curr.unlock();
50:  return result;
\end{SaveVerbatim}


\newcommand{\RemoveBody}{
    \begin{algorithmic}[1]
      \State $\prev, \curr := \locate(e)$
      \If {$\curr.\val = e$}
      \State $\aux := \curr.\tNext$
      \State $\prev.\tNext := \aux$
      \State $\result := \true$
      \Else
      \State $\result := \false$
      \EndIf
      \State $\prev.\unlock()$
      \State $\curr.\unlock()$
      \State \tbf{return} $\result$
      \Statex
    \end{algorithmic}
}

\newcommand{\RemovePrg}{
  \begin{minipage}[c]{3.9cm}
    \RemoveBody
  \end{minipage}
}


\newcommand{\RemoveFig}{
  \begin{minipage}[c]{3.9cm}
    \RemoveBody
    \label{fig:remove}
  \end{minipage}
}




%
% Figures for data structure
%
\newcommand{\DataStructuresGhostBody}{
	\begin{tabular}{cc}
		\renewcommand{\arraystretch}{0.4}
		$\begin{array}{l}
			\class \: \List \: \{ \\
			\mhs \Node \: \tList ;\\
			\hs{0.2} \fbox{ \begin{array}{l}
				\rgn \: r; \\
			\end{array}}\\
		\}
		\end{array}$ & \hs{2} $\begin{array}{l}
			\class \: \Node \: \{ \\
			\mhs \Value \: \val ;\\
			\mhs \Node \: \tNext ;\\
			\mhs \Lock \: \lock ;\\
		\}
	\end{array}$
	\end{tabular}
}

\newcommand{\DataStructuresGhostFig}{
\begin{minipage}[c]{6.5cm}
	\DataStructuresGhostBody
\label{fig:conclists:ghost}
\end{minipage}
}


%
% Figure for "locate" extended with ghost fields
%

\newcommand{\LocateGhostBody}{
	\begin{algorithmic}[1]
		\State $\prev := \Head$
		\State $\prev.\lock()$
		\State $\curr := \prev.\tNext$
		\State $\curr.lock()$
		\While {$\curr.\val < e$}
			\State $\prev.\unlock()$
			\State $\prev := \curr$
			\State $\curr := \curr.\tNext$
			\State $\curr.\lock()$
		\EndWhile
		\State \tbf{return} $(\prev, \curr)$
		\vspace{0.8cm}
	\end{algorithmic}
}


\newcommand{\LocateGhostFig}{
\begin{minipage}[c]{4.2cm}
	\LocateGhostBody
\label{fig:locate:ghost}
\end{minipage}
}


%
% Figure for "add" extended with ghost fields
%
\newcommand{\AddGhostBody}{
	\begin{algorithmic}[1]
		\State $\prev, \curr := \locate(e)$
		\If {$\curr.\val \neq e$}
			\State $\aux := \New \Node(e)$
			\State $\aux.\tNext := \curr$
			\State $\prev.\tNext := \aux$
			\Statex $\hs{0.7}\fbox{
				\begin{array}{l}
					l.r := l.r \cup \sreg{\aux} \\
				\end{array}}$
			\State $\result := \true$
		\Else
			\State $\result := \false$
		\EndIf
		\State $\prev.\unlock()$
		\State $\curr.\unlock()$
		\State \tbf{return} $\result$
	\end{algorithmic}
}


\newcommand{\AddGhostFig}{
\begin{minipage}[c]{4.2cm}
	\AddGhostBody
	\label{fig:add:ghost}
\end{minipage}
}


%
% Figure for "remove" extended with ghost fields
%
\newcommand{\RemoveGhostBody}{
		\begin{algorithmic}[1]
			\State $\prev, \curr := \locate(e)$
			\If {$\curr.\val = e$}
				\State $\aux := \curr.\tNext$
				\State $\prev.\tNext := \aux$
				\Statex $\hs{0.7}\fbox{
					\begin{array}{l}
						l.r := l.r - \sreg{\curr} \\
					\end{array}}$
				\State $\result := \true$
			\Else
				\State $\result := \false$
			\EndIf
			\State $\prev.\unlock()$
			\State $\curr.\unlock()$
			\State \tbf{return} $\result$
			\Statex
		\end{algorithmic}
}


\newcommand{\RemoveGhostFig}{
	\begin{minipage}[c]{4.3cm}
		\RemoveGhostBody
		\label{fig:remove:ghost}
  \end{minipage}
}



\begin{SaveVerbatim}{skiplist-data}
class Skiplist {
	Node* head;
	Node* tail;
	int maxLevel;

}
\end{SaveVerbatim}

\begin{SaveVerbatim}{skiplist-node-data}
class Node {
	Value v;
	Key k;
	Array<Node*>(4) next;
}
\end{SaveVerbatim}



==> figures/latex/slidesaux.tex <==
\newcommand{\VERT}{\phantom{|}}

\newcommand{\cemph}[1]{\textcolor{red}{\emph{#1}}}

%%% For LOLA
\newcommand{\IN}[1]{\textcolor{darkblue}{#1}}
\newcommand{\OUT}[1]{\textcolor{darkred}{#1}}
\newcommand{\DOM}[1]{\textcolor{darkgreen}{#1}}
\newcommand{\STRM}[1]{\textcolor{darkorange}{#1}}
\newcommand{\Input}{\IN{input}\xspace}
\newcommand{\Output}{\OUT{output}\xspace}
\newcommand{\Trigger}{\OUT{trigger}\xspace}
\newcommand{\Dbool}{\ensuremath{\text{\DOM{bool}}}\xspace}
\newcommand{\DboolThree}{\ensuremath{\text{\DOM{bool3}}}\xspace}
\newcommand{\DboolFour}{\ensuremath{\text{\DOM{bool4}}}\xspace}
\newcommand{\Dint}{\ensuremath{\text{\DOM{int}}}\xspace}
\newcommand{\Dset}{\ensuremath{\text{\DOM{set}}}\xspace}
\newcommand{\Delem}{\ensuremath{\text{\DOM{elem}}}\xspace}
\newcommand{\Keyword}[1]{\texttt{#1}\xspace}
\newcommand{\IFkw}{\Keyword{if}}
\newcommand{\THENkw}{\Keyword{then}}
\newcommand{\ELSEkw}{\Keyword{else}}
\newcommand{\IFk}{\ensuremath{\Keyword{if}\;\;}}
\newcommand{\THENk}{\ensuremath{\THENkw}\;\;}
\newcommand{\ELSEk}{\ensuremath{\ELSEkw\;\;}}

\newcommand{\sbool}{\textsf{bool}}
\newcommand{\sint}{\textsf{int}}
\newcommand{\sset}{\textsf{set}}
\newcommand{\ssetT}{\textsf{sestt}}
\newcommand{\selem}{\textsf{elem}}
\newcommand{\req}{\textit{req}}
\newcommand{\resp}{\textit{resp}}
\newcommand{\evresp}{\textit{evresp}}
\newcommand{\granted}{\textit{granted}}
\newcommand{\ok}{\textit{ok}}
\newcommand{\nreq}{\textit{nreq}}
\newcommand{\nresp}{\textit{nresp}}
\newcommand{\good}{\textit{good}}
\newcommand{\AlwaysGood}{\textit{G\_good}}
\newcommand{\END}{\textit{end}}
\newcommand{\pending}{\textit{pending}}
\newcommand{\reqid}{\textit{reqid}}
\newcommand{\respid}{\textit{respid}}
%\newcommand{\pending}{\textit{pending}}
\newcommand{\Int}{\text{Int}}

\newcommand{\hs}[1]{\hspace{#1cm}}
\newcommand{\mhs}{\hspace{0.5cm}}
\newcommand{\lsp}{\vspace{0.3cm}}

\newcommand{\StreamName}[1]{\textsf{#1}}
\newcommand{\Exp}[1]{\StreamName{E}_{\StreamName{#1}}}

\newcommand{\first}{\StreamName{first}}
\newcommand{\control}{\StreamName{control}}
\newcommand{\initial}{\StreamName{init}}
\newcommand{\last}{\StreamName{last}}
\newcommand{\test}[1]{\StreamName{test}_{\StreamName{#1}}}
\newcommand{\strFalse}{\StreamName{false}}
\newcommand{\strTrue}{\StreamName{true}}
\newcommand{\step}{\StreamName{step}}
\newcommand{\uniform}{\StreamName{uniform}}


\newcommand{\unique}{\StreamName{unique}}
\newcommand{\init}{\StreamName{initial}}
\newcommand{\transition}{\StreamName{transition}}
\newcommand{\accepting}{\StreamName{accepting}}

\newcommand{\prevEq}{\mathit{prev}_{\leq}}
\newcommand{\prev}{\mathit{prev}}

\newcommand{\cgreen}[1]{\textcolor{darkgreen}{#1}}
\newcommand{\cred}[1]{\textcolor{darkred}{#1}}
\newcommand{\cblue}[1]{\textcolor{darkblue}{#1}}
\newcommand{\corange}[1]{\textcolor{darkorange}{#1}}
\newcommand{\cmag}[1]{\textcolor{darkmagenta}{#1}}
\newcommand{\cmgreen}[1]{\textcolor{midgreen}{#1}}
\newcommand{\cmred}[1]{\textcolor{midred}{#1}}
\newcommand{\cmblue}[1]{\textcolor{midblue}{#1}}

% \newcommand{eventex}{
% \begin{tikzpicture}

% \matrix[column sep = 0.5em, draw] (m) {
%   \node[anchor = east] (m-1-2) {Event stream \texttt{e}};
%     \& \timing[name=m-2-3] at (0,-0.15) {ZZZ \n{0} Z \n{7} ZZZZ \n{2} ZZ \n{2} ZZZ \n{15} ZZ}; \\ 
  
%   \node[anchor = east] (m-1-3) {Signal \texttt{s}};  
%     \& \timing[name=m-2-2] at (0,-0.15) {4D{0}N(x1)4D{7}5D{2}2D{15}};\\
    
%   \node[anchor = east] (end-inputs) {Event stream \texttt{e2}}; 
%     \& \timing[name=m-2-3] at (0,-0.15) {ZZZZ \n{7} ZZZZ \n{2} ZZZZZ \n{15} ZZ}; \\  \\[0.5em]
% };
% \end{tikzpicture}
% }

\newcommand{\Time}{\ensuremath{\mathbb{T}}\xspace}
% \newcommand{\delay}{\ensuremath{\textit{delay}}\xspace}
\newcommand{\shift}{\ensuremath{\textit{shift}}\xspace}
\newcommand{\within}{\ensuremath{\textit{within}}\xspace}


\newcommand{\op}[1]{\operatorname{#1}}
\newcommand{\peek}{\op{peek}}
%\newcommand{\pop}{\op{pop}}
%\newcommand{\last}{\op{last}}
\newcommand{\tim}{\op{time}}
% \newcommand{\Val}{\op{value}}
\newcommand{\emit}{\op{emit}}
\newcommand{\dequeue}{\op{dequeue}}
\newcommand{\progress}{\op{progress}}

\newcommand{\plotwidth}{32mm}
\newcommand{\plotheight}{20mm}


==> figures/latex/solidity-highlighting.tex <==
% Copyright 2017 Sergei Tikhomirov, MIT License
% https://github.com/s-tikhomirov/solidity-latex-highlighting/

\usepackage{listings}
\usepackage[dvipsnames]{xcolor}

\definecolor{verylightgray}{rgb}{.97,.97,.97}

\lstdefinelanguage{Solidity}{
	keywords=[1]{anonymous, assembly, assert, balance, break, call, callcode, case, catch, class, constant, continue, constructor, contract, debugger, default, delegatecall, delete, do, else, emit, event, experimental, export, external, false, finally, for, function, gas, if, implements, import, in, indexed, instanceof, interface, internal, is, length, library, log0, log1, log2, log3, log4, memory, modifier, new, payable, pragma, private, protected, public, monitor_storage, pure, push, require, return, returns, revert, selfdestruct, send, solidity, storage, struct, suicide, super, switch, then, this, throw, transfer, true, try, typeof, using, value, view, while, with, addmod, ecrecover, keccak256, mulmod, ripemd160, sha256, sha3}, % generic keywords including crypto operations
	keywordstyle=[1]\color{blue}\bfseries,
	keywords=[2]{set,address, bool, byte, bytes, bytes1, bytes2,
	bytes3, bytes4, bytes5, bytes6, bytes7, bytes8, bytes9,
	bytes10, bytes11, bytes12, bytes13, bytes14, bytes15, bytes16,
	bytes17, bytes18, bytes19, bytes20, bytes21, bytes22, bytes23,
	bytes24, bytes25, bytes26, bytes27, bytes28, bytes29, bytes30,
	bytes31, bytes32, enum, int, int8, int16, int24, int32, int40,
	int48, int56, int64, int72, int80, int88, int96, int104,
	int112, int120, int128, int136, int144, int152, int160,
	int168, int176, int184, int192, int200, int208, int216,
	int224, int232, int240, int248, int256, mapping, string, elem,
	uint, uint8, uint16, uint24, uint32, uint40, uint48, uint56,
	uint64, uint72, uint80, uint88, uint96, uint104, uint112,
	uint120, uint128, uint136, uint144, uint152, uint160, uint168,
	uint176, uint184, uint192, uint200, uint208, uint216, uint224,
	uint232, uint240, uint248, uint256, var, void, ether, finney,
	szabo, wei, days, hours, minutes, seconds, weeks, years, map,
        txId},	% types; money and time units
	keywordstyle=[2]\color{teal}\bfseries,
	keywords=[3]{block, blockhash, coinbase, difficulty, gaslimit,
	number, timestamp, msg, gas, sender, sig, value, now, tx,
	gasprice, origin, add, epochinc, get, setminus, emptyset,
	system, first, fail, commit, undecided, failmap, queue, ustore, isSelfOnly, gen_op,
	verdict, monitor, tx_id, preCommit, abort, preAbort},	% environment variables
	keywordstyle=[3]\color{violet}\bfseries,
	keywords=[4]{init, term, begin,end, upon, timeout},
	keywordstyle=[4]\color{BrickRed}\bfseries,
	identifierstyle=\color{black},
	sensitive=false,
	comment=[l]{//},
	morecomment=[s]{/*}{*/},
	commentstyle=\color{gray}\ttfamily,
	stringstyle=\color{red}\ttfamily,
	morestring=[b]',
	morestring=[b]"
}

\lstset{
	language=Solidity,
        %% backgroundcolor=\color{verylightgraywhite},
	backgroundcolor=\color{white},
	extendedchars=true,
%	basicstyle=\footnotesize\ttfamily,
	basicstyle=\footnotesize\ttfamily,
	showstringspaces=false,
	showspaces=false,
	numbers=left,
	numberstyle=\footnotesize,
	numbersep=9pt,
	tabsize=2,
	breaklines=true,
	showtabs=false,
	captionpos=b
}


==> figures/latex/theories.tex <==
%
% T_{fSeq} to T_{path} Auxiliary Functions
%
\newcommand{\TPathFig}{
\renewcommand{\arraystretch}{1}
\centering
\begin{tabular}{|c|}
\hline
$\fApp : \sSeq \times \sSeq \to \sSeq$ \\
\hline
$\fApp (\fNil, l) = l$ \\
$\fApp(\fCons(a,l), l') = \fCons(a, \fApp(l, l'))$ \\
\hline
\hline
$\fSeqToSet : \sSeq \to \sSet$ \\
\hline
$\fSeqToSet (\fNil) = \emptyset$ \\
$\fSeqToSet (\fCons(a,l)) = \{ a \} \cup \fSeqToSet(l)$ \\
\hline
\hline
$\fIsPath : \sSeq$ \\
\hline
$\fIsPath(\fNil)$ \\
$\fIsPath(\fCons(a, \fNil))$ \\
$\{a\} \nsubseteq \fSeqToSet(l) \land \fIsPath(l) \Impl
	\fIsPath(\fCons(a,l))$ \\
\hline
\hline
$\fLast : \sSeq \to \sAddr$ \\
\hline
$\fLast(\fCons(a, \fNil)) = a$ \\
$l \neq \fNil \Impl \fLast(\fCons(a, l)) = \fLast(l)$ \\
\hline
\hline
$\pIsReachK : \sMem \times \sAddr \times \sAddr \times \sLevelK$ \\
\hline
$\pIsReachK(m, a, a, l)$ \\
$m[a].\fNext[l] = a' \land \pIsReach(m, a', b, l)
	\Impl \pIsReach(m, a, b, l)$ \\
\hline
\hline
$\pIsReachKP : \sMem \times \sAddr \times \sAddr \times \sLevelK
	\times \sSeq$ \\
\hline
$\pIsReachKP(m, a, a, l, \fNil)$ \\
$m[a].\fNext[l] = a' \land \pIsReachP(m, a', b, l, p) \Impl
	\pIsReachP(m, a, b, l, \fCons(a, p))$ \\
\hline
\hline
$\fFirstMarked : \sMem \times \sSeq \times \sLevelK \times \sAddr$ \\
\hline
$\fFirstMarked (m, \fNil, l, \fNull)$ \\
$p \neq \fNil \land p = \fCons(j, q) \land m[j].\fLockID[l] \neq \oslash
	\Impl \fFirstMarked(m, p, l, j)$ \\
$p \neq \fNil \land p = \fCons(j, q) \land m[j].\fLockID[l] = \oslash
	\land \fFirstMarked(m, q, l, i)
		\Impl \fFirstMarked(m, p, l, i)$ \\
\hline
\hline
$\pOrdPath : \sMem \times \sSeq$ \\
\hline
$\pOrdPath(h, \fNil)$ \\
$h[a].\fNext[\fLevel{0}] = a' \land h[a].\fKey \pOrd h[a'].\fKey \land
	p = \fCons(a, q) \land \pOrdPath(h, q) \Impl \pOrdPath(h, p)$ \\
\hline
\end{tabular}
}


%
% TLLpL Auxiliary Functions
%
\newcommand{\AuxiliaryFunctions}{
\centering
\begin{tabular}{|c|}
\hline
$\List : \sMem \times \sAddr \times \sSet$ \\
\hline
$\begin{array}{lcl}
	\List(h,a,r) & \Iff & \fNull \in \fAddrToSet(h, a)
		\land r = \fPathToSet(\fGetp(h, a, \fNull)) \\
\end{array}$\\
\hline
\hline
$\fa : \sMem \times \sAddr \to \sPath$ \\
\hline
$\fa(h,n) = \begin{cases}
		\fEpsilon & \trm{if } n = \fNull \\
		\fGetp(h, h[n].\fNext, \fNull) & \trm{if } n \neq \fNull \\
		\end{cases}$ \\
\hline
%
% Begin: Function removed to reduce space
%
%\hline
%$\fb : \sMem \times \sAddr \times \sAddr \times \sPath$ \\
%\hline
%$\begin{array}{lcl}
%\fb(h, n, m, p) & \Iff & (n = \fNull \land p = \fEpsilon)
%	\lor \; \big(n \neq \fNull \land \pReach(h,n,m,\tilde{p})\\
%		&& \hs{3.5} \land \; m = \fNull
%			\Impl \pAppend(p, \fNull, \tilde{p}) \\
%		&& \hs{3.5} \land \; m \neq \fNull
%			\Impl \pAppend(p, [m], \tilde{p}) \big) \\
%\end{array}$ \\
%\hline
\hline
$\LastMarked : \sMem \times \sPath \to \sAddr$ \\
\hline
$\LastMarked(m, p) = \fFirstLocked(m, \fRev(p))$ \\
\hline
\hline
$\NoMarks : \sMem \times \sPath$ \\
\hline
$\NoMarks(m,p) \Iff \fFirstLocked(m,p) = \fNull$ \\
\hline
\hline
$\SomeMark : \sMem \times \sPath$ \\
\hline
$\SomeMark(m,p) \Iff \fFirstLocked(m,p) \neq \fNull$ \\
\hline
\end{tabular}
}



%
% TSLK Signature
%
\newcommand{\TSLKSignature}{
\centering
\begin{tabular}{|c|c|c|c|}
\hline
Signature & \hs{0.1} Sorts \hs{0.1} & Functions & Predicates \\
\hline
\hline
\sigLevelK &
	$\begin{array}{c}
		\sLevelK
	\end{array}$ &
	$\begin{array}{lcl}
		0,1, \ldots, \K-1 & : & \sLevelK \\
	\end{array}$ &
	$\begin{array}{lcl}
		< : \sLevelK \times \sLevelK
	\end{array}$\\
\hline
\sigOrd &
	$\begin{array}{c}
		\sOrd
	\end{array}$ &
	$\begin{array}{lcl}
		\fZero & : & \sOrd \\
		\fInfty & : & \sOrd \\
	\end{array}$ &
	$\begin{array}{lcl}
		\pOrd & : & \sOrd \times \sOrd \\
	\end{array}$ \\
\hline
\sigThId &
	$\begin{array}{c}
		\sThId
	\end{array}$ &
	$\begin{array}{lcl}
		\oslash & : & \sThId \\
	\end{array}$ & \\
\hline
\hline
\sigCells &
	$\begin{array}{c}
		\sCell \\ \sElem \\ \sOrd \\ \sAddr \\ \sThId
	\end{array}$ &
	$\begin{array}{lcl}
		\fError & : & \sCell \\
		\fMkcell & : & \sElem \times \sOrd \times \sAddr^{\K}
			\times \sThId^{\K} \to \sCell \\
		\_.\fData & : & \sCell \to \sElem \\
		\_.\fKey & : & \sCell \to \sOrd \\
		\_.\fNext \lbrack \_ \rbrack & : & \sCell \times \sLevelK
			\to \sAddr \\
		\_.\fLockID \lbrack \_ \rbrack & : & \sCell
			\times \sLevelK \to \sThId \\
		\_.\fLock \lbrack \_ \rbrack & : & \sCell \times \sLevelK	
			\to \sThId \to \sCell \\
		\_.\fUnlock \lbrack \_ \rbrack & : & \sCell
			\times \sLevelK \to \sCell \\
	\end{array}$ & \\
\hline
\sigMemory &
	$\begin{array}{c}
		\sMem \\ \sAddr \\ \sCell
	\end{array}$ &
	$\begin{array}{lcl}
		\fNull & : & \sAddr \\
		\_[\_] & : & \sMem \times \sAddr \to \sCell \\
		\fUpd & : & \sMem \times \sAddr \times \sCell \to \sMem
	\end{array}$ & \\
\hline
\sigReach &
	$\begin{array}{c}
		\sMem \\ \sAddr \\ \sPath
	\end{array}$ &
	$\begin{array}{lcl}
		\fEpsilon & : & \sPath \\
		\lbrack \_ \rbrack & : & \sAddr \to \sPath
	\end{array}$ &
	$\begin{array}{lcl}
		\pAppend & : & \sPath \times \sPath \times \sPath \\
		\pReachK & : & \sMem \times \sAddr \times \sAddr \\
				&& \mhs \times \; \sLevelK \times \sPath \\
	\end{array}$ \\
\hline
\hline
\sigSets &
	$\begin{array}{c}
		\sAddr \\ \sSet
	\end{array}$ &
	$\begin{array}{lcl}
		\emptyset & : & \sSet \\
		\{ \_ \} & : & \sAddr \to \sSet \\
		\cup, \cap, \setminus & : & \sSet \times \sSet \to \sSet
	\end{array}$ &
	$\begin{array}{lcl}
		\in & : & \sAddr \times \sSet \\
		\subseteq & : & \sSet \times \sSet
	\end{array}$ \\
\hline
\sigSetsT &
	$\begin{array}{c}
		\sThId \\ \sSetT
	\end{array}$ &
	$\begin{array}{lcl}
		\stEmpty & : & \sSetT \\
		\stSingle{\_} & : & \sThId \to \sSetT \\
		\stCup, \stCap, \stSubst & : & \sSetT \times \sSetT \to \sSetT
	\end{array}$ &
	$\begin{array}{lcl}
		\stIn & : & \sThId \times \sSetT \\
		\stSubset & : & \sSetT \times \sSetT
	\end{array}$ \\
\hline
\sigMrgn &
	$\begin{array}{c}
		\sMrgn, \\ \sAddr \\ \sLevelK
	\end{array}$ &
	$\begin{array}{lcl}
		\mrgnEmpty & : & \sMrgn \\
		\mrgnSingle{\_, \_} & : & \sAddr \times \sLevelK \to \sMrgn \\
		\mrgnCup, \mrgnCap, \mrgnMinus & : & \sMrgn \times \sMrgn
			\to \sMrgn
	\end{array}$ &
	$\begin{array}{lcl}
		\mrgnIn & : & \sAddr \times \sLevelK \times \sMrgn \\
		\mrgnSubset & : & \sMrgn \times \sMrgn \\
		\mrgnDisj & : & \sMrgn \times \sMrgn
	\end{array}$ \\
\hline
\hline
\sigBridge &
	$\begin{array}{c}
		\sMem \\ \sAddr \\ \sSet \\ \sPath
	\end{array}$ &
	$\begin{array}{lcl}
		\fPathToSet & : & \sPath \to \sSet \\
		\fAddrToSetK & : & \sMem \times \sAddr \times \sLevelK
			\to \sSet \\
		\fGetpK & : & \sMem \times \sAddr \times \sAddr \times
			\sLevelK \to \sPath \\
		\fFirstLockedK & : & \sMem \times \sPath \times \sLevelK
			\to \sAddr
	\end{array}$ &
	$\begin{array}{lcl}
		\pOrdList & : & \sMem \times \sPath \\
	\end{array}$ \\
\hline
\end{tabular}
}


%
% TSLK Interpretations
%
\newcommand{\TSLKInterpretationsOne}{
\centering
\begin{tabular}{|c|p{10.5cm}|}
\hline
\multicolumn{2}{|c|}{Interpretation of sort symbols: \sAddr, \sElem, 
\sThId, \sLevelK, \sOrd, \sCell, \sMem, \sPath, \sSet, \sSetT and \sMrgn}
\\
\hline
\hline
\multicolumn{2}{|l|}{
Each sort $\sigma$ in \sigTSLK is mapped to a non-empty set $\Ais{\sigma}$ 
such that:} \\
\multicolumn{2}{|l|}{
\begin{tabular}{clcl}
	(a) &$\Ais{\sAddr}$ and $\Ais{\sElem}$ are discrete sets &
	(b) &$\Ais{\sThId}$ is a discrete set containing symbol $\oslash$ \\
	(c) &$\Ais{\sLevelK}$ is the finite collection 0,\ldots,\K-1 &
	(d) &$\Ais{\sOrd}$ is a collection of total ordered identifiers \\
	(e) &$\Ais{\sCell} = \Ais{\sElem} \times \Ais{\sOrd} \times 
		\Ais{\sAddr}^{\K} \times \Ais{\sThId}^{\K}$ &
	(f) &$\Ais{\sMem} = \Ais{\sCell}^{\Ais{\sAddr}}$ \\
	(g) &$\Ais{\sPath}$ is the set of all finite sequences of &
	(h) &$\Ais{\sSet}$ is the power-set of $\Ais{\sAddr}$ \\
		& \hs{0.5} (pairwise) distinct elements of $\Ais{\sAddr}$ &
	(i) &$\Ais{\sSetT}$ is the power-set of $\Ais{\sThId}$ \\
	(j) &$\Ais{\sMrgn}$ is the power-set of
		$\Ais{\sAddr} \times \Ais{\sLevelK}$ &
\end{tabular}
} \\
\hline
\hline
Signature & Interpretation \\
\hline
%\hline
%\sigLevelK &
%	\begin{tabular}{p{9.7cm}}
%		$\inter{\fLevel{i}}{\Ai} \neq \inter{\fLevel{j}}{\Ai}$
%			when $i \neq j$
%	\end{tabular} \\
\hline
\sigOrd &
	\begin{tabular}{p{9.7cm}}
		$x \inter{\pOrd}{\Ai} y \land y \inter{\pOrd}{\Ai} x
			\Impl x = y$ for any $x, y \in \Ais{\sOrd}$ \\
		$x \inter{\pOrd}{\Ai} y \land y \inter{\pOrd}{\Ai} z
			\Impl x \inter{\pOrd}{\Ai} z$
			for any $x, y, z \in \Ais{\sOrd}$ \\
		$x \inter{\pOrd}{\Ai} y \lor y \inter{\pOrd}{\Ai} x$
			for any $x, y \in \Ais{\sOrd}$ \\
		$\inter{\fZero}{\Ai} \inter{\pOrd}{\Ai} x \land
		x \inter{\pOrd}{\Ai} \inter{\fInfty}{\Ai}$
			for any $x \in \Ais{\sOrd}$ \\
%		$x \neq \inter{\fInfty}{\Ai} \Impl
%			x \inter{\pOrd}{\Ai} \inter{\fSucc}{\Ai}(x)$
%			for any $x \in \Ais{\sOrd}$ \\
	\end{tabular} \\
\hline
\hline
\sigCells &
	\begin{tabular}{p{11.5cm}}
		\begin{compactitem}
		\item $\inter{\fMkcell}{\Ai} (e, k, a_0, \ldots, a_{\K-1},
						t_0, \ldots, t_{\K-1}) =
			\langle e, k, a_0, \ldots, a_{\K-1},
				t_0, \ldots, t_{\K-1} \rangle$
			for each
			$e \in \Ais{\sElem}$, $i \in \Ais{\sOrd}$,
			$a_0, \ldots, a_{\K-1} \in \Ais{\sAddr}$
			and $t_0, \ldots, t_{\K-1} \in \Ais{\sThId}$
		\item $\langle e, k, \vect{a}, \vect{t} \rangle
				.\inter{\fData}{\Ai} = e$
			for each $e \in \Ais{\sElem}$,
			$k \in \Ais{\sOrd}$,
			$\vect{a} \in \Ais{\sAddr}^{\K}$
			and $\vect{t} \in \Ais{\sThId}^{\K}$
		\item $\langle e, k, \vect{a}, \vect{t} \rangle
				.\inter{\fKey}{\Ai} = k$
			for each $e \in \Ais{\sElem}$,
			$k \in \Ais{\sOrd}$,
			$\vect{a} \in \Ais{\sAddr}^{\K}$
			and $\vect{t} \in \Ais{\sThId}^{\K}$
		\item $\langle e, k, a_0, \ldots, a_{\K-1}, \vect{t} \rangle
				.\inter{\fNext}{\Ai}[j] = a_j$
			for each $e \in \Ais{\sElem}$,
			$k \in \Ais{\sOrd}$,
			$a_0 \ldots, a_{\K-1} \in \Ais{\sAddr}$,
			$j \in \Ais{\sLevelK}$
			and $\vect{t} \in \Ais{\sThId}^{\K}$ and
		\item $\langle e, k, \vect{a}, t_0, \ldots, t_{\K-1} \rangle
				.\inter{\fLockID}{\Ai}[j] = t_{j}$
			for each $e \in \Ais{\sElem}$,
			$k \in \Ais{\sOrd}$,
			$\vect{a} \in \Ais{\sAddr}^{\K}$,
			$j \in \Ais{\sLevelK}$
			and $t_0, \dots, t_{\K-1} \in \Ais{\sThId}$
		\item $\langle e, k, \vect{a}, t_0, \ldots, t_{\K-1} \rangle
				.\inter{\fLock}{\Ai}[j](t') =
			\langle e, k, \vect{a},
				t_0, \ldots, t_{j-1}, t',
				t_{j+1}, \ldots, t_{\K-1}
			\rangle$
			for each $e \in \Ais{\sElem}$,
			$k \in \Ais{\sOrd}$,
			$\vect{a} \in \Ais{\sAddr}^{\K}$,
			$j \in \Ais{\sLevelK}$
			and $t_0, \ldots, t_{\K-1}, t' \in \Ais{\sThId}$
		\item $\langle e, k, \vect{a}, t_0, \ldots, t_{\K-1} \rangle
				.\inter{\fUnlock}{\Ai}[j] =
			\langle e, k, \vect{a},
				t_0, \ldots, t_{j-1}, \oslash,
				t_{j+1}, \ldots, t_{\K-1}
			\rangle$
			for each $e \in \Ais{\sElem}$,
			$k \in \Ais{\sOrd}$,
			$\vect{a} \in \Ais{\sAddr}^{\K}$,
			$j \in \Ais{\sLevelK}$
			and $t_0, \ldots, t_{\K-1} \in \Ais{\sThId}$
		\item $\inter{\fError}{\Ai}.\inter{\fNext}{\Ai} =
			\inter{\fNull}{\Ai}$
		\end{compactitem}
	\end{tabular} \\
\hline
\sigMemory &
	\begin{tabular}{p{9.7cm}}
		\begin{compactitem}
		\item $m\inter{[a]}{\Ai} = m(a)$ for each $m \in \Ais{\sMem}$
			and $a \in \Ais{\sAddr}$
		\item $\inter{\fUpd}{\Ai}(m,a,c) = m_{a \mapsto c}$ for each
			$m \in \Ais{\sMem}$, $a \in \Ais{\sAddr}$ and
			$c \in \Ais{\sCell}$
		\item $\inter{m}{\Ai}(\inter{\fNull}{\Ai}) = 
			\inter{\fError}{\Ai}$
			for each $m \in \Ais{\sMem}$
		\end{compactitem}
	\end{tabular} \\
\hline
\sigReach &
	\begin{tabular}{p{11cm}}
		\begin{compactitem}
		\item $\inter{\fEpsilon}{\Ai}$ is the empty sequence
		\item $\inter{[i]}{\Ai}$ is the sequence containing $i \in 
			\Ais{\sAddr}$ as the only element
		\item $\left(\left[i_1,\ldots, i_n\right], \left[j_1, \ldots, 
			j_m\right], \left[i_1,\ldots, i_n, j_1,
				\ldots, j_m\right]
			\right) \in \inter{\pAppend}{\Ai}$ iff $i_k$
		and $j_l$ are all distinct
		\item $(m, \aInit, \aEnd, l, p) \in \inter{\pReachK}{\Ai}$
			iff $\aInit=\aEnd$ and $p = \fEpsilon$, or
		there exist addresses $a_1, \ldots, a_n \in \Ais{\sAddr}$ such 
		that:
		\end{compactitem} \\
		\hs{1.5} $\begin{array}{ll}
			\trm{(a) } p = [a_1, \ldots, a_n]  \phantom{aaaa}&
			\trm{(c) } m(a_r).\inter{\fNext}{\Ai}[l]
				= a_{r+1}, \trm{for } 1 \leq r < n \\
			\trm{(b) } a_1 = \aInit &
			\trm{(d) } m(a_n).\inter{\fNext}{\Ai}[l]
				= \aEnd
		\end{array}$
	\end{tabular} \\
\hline
\hline
\sigSets &
	\begin{tabular}{p{11cm}}
		The symbols $\emptyset$, $\{ \_ \}$, $\cup$, $\cap$, 
		$\setminus$, $\in$ and $\subseteq$ are interpreted 
according to
		their standard interpretation over sets of addresses.
	\end{tabular} \\
\hline
\sigSetsT &
	\begin{tabular}{p{11cm}}
		The symbols $\stEmpty$, $\stSingle{\_}$, $\stCup$, $\stCap$, 
		$\stSubst$, $\stIn$ and $\stSubset$ are interpreted according
		to their standard interpretation over sets of thread
		identifiers.
	\end{tabular} \\
\hline
\end{tabular}
}


\newcommand{\TSLKInterpretationsTwo}{
\centering
\begin{tabular}{|c|p{11.7cm}|}
\hline
Signature & Interpretation \\
\hline
\hline
\sigMrgn &
	\begin{tabular}{p{11cm}}
		\begin{compactitem}
		\item $\mrgnEmptyI{\Ai} = \emptyset$
		\item $\mrgnSingleI{a,j}{\Ai} = \{ (a,j) \}$
			for each $a \in \Ais{\sAddr}$
			and $j \in \Ais{\sLevelK}$
		\item $m_1 \mrgnCupI{\Ai} m_2 = m_1 \cup m_2$
			for each $m_1, m_2 \in \Ais{\sMrgn}$
		\item $m_1 \mrgnCapI{\Ai} m_2 = m_1 \cap m_2$
			for each $m_1, m_2 \in \Ais{\sMrgn}$
		\item $m_1 \mrgnMinusI{\Ai} m_2 = m_1 \setminus m_2$
			for each $m_1, m_2 \in \Ais{\sMrgn}$
		\item $m_1 \mrgnSubsetI{\Ai} m_2 \Iff m_1 \subseteq m_2$
			for each $m_1, m_2 \in \Ais{\sMrgn}$
		\item $(a,j) \mrgnInI{\Ai} m \Iff (a,j) \in m$
			for each $a \in \Ais{\sAddr}$,
			$j \in \Ais{\sLevelK}$ and $m \in \Ais{\sMrgn}$
		\item $m_1 \mrgnDisjI{\Ai} m_2 \Iff m_1 \mrgnCapI{\Ai} m_2
			= \mrgnEmptyI{\Ai}$
			for each $m_1, m_2 \in \Ais{\sMrgn}$
		\end{compactitem}
	\end{tabular} \\
\hline
\hline
\sigBridge &
	\begin{tabular}{p{11cm}}
		\begin{compactitem}
		\item $\inter{\fPathToSet}{\Ai}(p) = \{ a_1, \ldots, 
			a_n\}$ for $p = [a_1, \ldots, a_n] \in
			\Ais{\sPath}$
		\item $\inter{\fAddrToSetK}{\Ai}(m, a, l) = \big\{
			a' \in \Ais{\sAddr} \:|\: \exists p \in 
			\Ais{\sPath}$ s.t. $(m,a,a',l,p) \in \pReachK
			\big\}$
		\item $\inter{\fGetpK}{\Ai}(m,\aInit,\aEnd,l) =
			\begin{cases}
				p & \text{if } (m,\aInit,\aEnd,l,p)
					\in \inter{\pReachK}{\Ai} \\
				\fEpsilon & \text{otherwise}
			\end{cases}$
		\end{compactitem} \\
			\hspace{1cm} for each $m \in \Ais{\sMem}$,
			$p \in \Ais{\sPath}$, $l \in \Ais{\sLevelK}$
			and $\aInit, \aEnd \in \Ais{\sAddr}$
		\begin{compactitem}
		\item $\inter{\fFirstLocked}{\Ai}\left(m,[a_1, \ldots,
			a_n], l \right) =\left\{
			\begin{array}{ll}
			a_k &
			\trm{if there is } 1 \leq k \leq n \trm{ such that } \\
			& \trm{for all } 1 \leq j < k,
				m[a_j].\fLockID[l] = \oslash \\
			& \trm{and } m[a_k].\fLockID[l] \neq \oslash \\
			\fNull & \trm{otherwise }
			\end{array}
			\right.$
		\item $\inter{\pOrdList}{\Ai}\left(m,p \right)$
			iff $p=\fEpsilon$ or $p = \lbrack a \rbrack$ or
			$p = [a_1, \ldots, a_n]$ with $n \geq 2$ and
			$m(a_i).\inter{\key}{\Ai} \pOrd
				m(a_{i+1}).\inter{\key}{\Ai}$
			for all $1 \leq i < n$,
			for any $m \in \Ais{\sMem}$
		\end{compactitem}
	\end{tabular} \\
\hline
\end{tabular}
}


==> figures/latex/vpl-macros.tex <==
\newcommand{\val}[1]{\ensuremath{[\![ #1 ]\!]}}
\newcommand{\der}[1]{\ensuremath{{\mathop{{ %
            \longrightarrow}}\limits^{{#1}}}\!}} %
\newcommand \tpl[1]{\langle #1 \rangle}
%\newcommand{\RE}{\textsf{RE}\xspace}
\newcommand{\NVPA}{\textsf{NVPA}\xspace}
\newcommand{\VPA}{\textsf{VPA}\xspace}
\newcommand{\NFA}{\textsf{NFA}\xspace}
\newcommand{\VPL}{\textsf{VPL}\xspace}
\newcommand{\CARET}{\textsf{CaRet}\xspace}
\newcommand{\VPLs}{\textsf{VPL}s\xspace}
\newcommand{\VRL}{\textsf{VRL}\xspace}
\newcommand{\VRE}{\textsf{VRE}\xspace}
\newcommand{\EMSO}{\textsf{MSO$_{\mu}$}\xspace}
\newcommand{\MSO}{\textsf{MSO}\xspace}
\newcommand{\XML}{\textsf{XML}\xspace}

\newcommand{\EXPTIME}{{\sffamily EXPTIME}\xspace}

\newcommand{\WM}{\ensuremath{\mathit{WM}}\xspace}
\newcommand{\MR}{\ensuremath{\mathit{MR}}\xspace}
\newcommand{\MC}{\ensuremath{\mathit{MC}}\xspace}
\newcommand{\SWM}{\ensuremath{\mathit{MWM}}\xspace}
\newcommand{\Pu}{\ensuremath{\mathcal{P}}\xspace}
%\newcommand{\Lang}{\ensuremath{\mathcal{L}}\xspace}
\newcommand{\Au}{\ensuremath{\mathcal{A}}}
\newcommand{\Msubst}{$M$-substitution\xspace}
\newcommand{\Mclosure}{$M$-closure\xspace}
\newcommand{\Sclosure}{$S$-closure\xspace}


\newcommand{\Stilde}{\widetilde{\Sigma}\xspace}
\newcommand{\Scall}{\Sigma_{\mathit{call}}\xspace}
\newcommand{\Sret}{\Sigma_{\mathit{ret}}\xspace}
\newcommand{\Sint}{\Sigma_{\mathit{int}}\xspace}

\newcommand{\SubstOp}[1]{\mathrel{\curvearrowleft_{#1}}}
\newcommand{\SubstBox}{\SubstOp{\Box}}
\newcommand{\MClos}[2]{#1^{\SubstOp{#2}}}
\newcommand{\LangClos}{\MClos{\Lang}{\Box}}
\newcommand{\SClos}[2]{{#1}^{\circlearrowleft_{#2}}}
\newcommand{\SClosure}[1]{\SClos{#1}{\Box}}
\newcommand{\LangSClos}{\SClos{\Lang}{\Box}}



%\newcommand{\DefinedAs}{\,\stackrel{\text{def}}{=}\,}

%\newcommand{\DefOR}{\ensuremath{\;\;\;\big|\;\;\;}}
\newcommand{\DefORmini}{\ensuremath{\;\;\big|\;\;}}

\newcommand{\details}[1]{}

\newcommand{\Outcm}{c\,b\,r}
\newcommand{\UOutcm}{\underline{\Outcm}}

\newcommand{\LSet}{R}
\newcommand{\SSet}{S}

\newcommand{\qin}{\ensuremath{q_{\textit{in}}}}
